Making Machine Learning Datasets and Models FAIR for HPC: A Methodology and Case Study

The FAIR Guiding Principles aim to improve the findability, accessibility, interoperability, and reusability of digital content by making them both human and machine actionable. However, these principles have not yet been broadly adopted in the domain of machine learning-based program analyses and optimizations for High-Performance Computing (HPC). In this paper, we design a methodology to make HPC datasets and machine learning models FAIR after investigating existing FAIRness assessment and improvement techniques. Our methodology includes a comprehensive, quantitative assessment for elected data, followed by concrete, actionable suggestions to improve FAIRness with respect to common issues related to persistent identifiers, rich metadata descriptions, license and provenance information. Moreover, we select a representative training dataset to evaluate our methodology. The experiment shows the methodology can effectively improve the dataset and model's FAIRness from an initial score of 19.1% to the final score of 83.0%.

==> TEML'22 FAIRness-Extended-arXiv/FAIRness.tex <==
%We give some background information for the FAIR Guiding Principles in this section.
%\subsection{FAIR Guiding Principles (1 page)}
\textbf{FAIR Guiding Principles: }
With a massive amount of data generated and collected in research activities, the scientific communities are pursuing good data management and data stewardship to have high quality digital publications that can simplify data discovery, evaluation, and reuse in downstream studies.  
%To achieve such goal, it requires a clear definition of ``good data management" and guidance for data publishers to follow.
The FAIR Guiding Principles, standing for findable, accessible, interoperable and reusable,  were jointly prepared by representatives and interested stakeholder groups
as guidelines for data management and stewardship~\cite{wilkinson2016fair}. 

\begin{comment}

Table~\ref{tab:FAIR-principle} lists the refined definitions of the FAIR Guiding Principles. These independent but related principles together define the data characteristics to improve the data discoverability and reusability.
Instead of serving as specifications to enforce the implementations, they are meant to guide data generators,  researchers, and stewards to create a FAIR data environment.

\begin{table*}[ht]
\begin{center}
\begin{tabular}{|p{0.06\textwidth}|p{0.94\textwidth}|}
    \hline
    \multicolumn{2}{|l|}{\textbf{F: To be Findable}}\\ \hline
    F1 & (Meta)data are assigned a globally unique and persistent identifier\\ \hline
    F2 & Data are described with rich metadata\\ \hline
    F3 & Metadata clearly and explicitly include the identifier of the data they describe\\ \hline
    F4 & (Meta)data are registered or indexed in a searchable resource\\ \hline
    \multicolumn{2}{|l|}{\textbf{A: To be Accessible}}\\ \hline
    A1 & (Meta)data are retrievable by their identifier using a standardized communications protocol\\ \hline
    A1.1 & The protocol is open, free, and universally implementable\\ \hline
    A1.2 & The protocol allows for an authentication and authorization procedure, where necessary\\ \hline
    A2 & Metadata are accessible, even when the data are no longer available\\ \hline
    \multicolumn{2}{|l|}{\textbf{I: To be Interoperable}}\\ \hline
    I1 & (Meta)data use a formal, accessible, shared, and broadly applicable language for knowledge representation \\ \hline
    I2 & (Meta)data use vocabularies that follow FAIR principles \\ \hline
    I3 & (Meta)data include qualified references to other (meta)data \\ \hline
    \multicolumn{2}{|l|}{\textbf{R: To be Reusable}}\\ \hline
    R1 & (Meta)data are richly described with a plurality of accurate and relevant attributes\\ \hline
    R1.1 & (Meta)data are released with a clear and accessible data usage license\\ \hline
    R1.2 & (Meta)data are associated with detailed provenance\\ \hline
    R1.3 & (Meta)data meet domain-relevant community standards\\ \hline
\end{tabular}
\end{center}
\caption{FAIR Guiding Principles}
\label{tab:FAIR-principle}
\end{table*}

\end{comment}

%\subsection{FAIRness Evaluation (0.75 page)}
\noindent\textbf{FAIRness Evaluation:}
%To bring the FAIR principles into practice, 
FAIRness evaluation plays an important role by providing assessments to assist data generators and stewards to improve the data FAIRness. 
%Prior to the debut of the FAIR principles, 
%The term FAIR and the concept of ``levels of FAIRness" were first appeared at a Lorentz Workshop ``Jointly Designing a Data FAIRport" in 2014.
%\todo{To Pei-Hung: who proposed the evaluation? How are they related to GO FAIR or FORCE11? Is this the only authoritative evaluation in the field?} 
\begin{comment}
A 4-level of data FAIRness was presented by FORCE11 with the following definitions~\cite{FAIRPrinciples}: 
Level 1) Each data object has a Persistent Identifier (PID) and intrinsic FAIR metadata. Level 2) Each data object has `user defined' (and updated) metadata to give rich provenance in FAIR format of the data.
%    \item[] Level 2: user defined (and updated) metadata is provided to give rich provenance in FAIR format of the data. The metadata can also be seen as the FAIR annotation to describe what happened to the data, what it has been used for, can be used for etc.
    Level 3) The data elements themselves in the data objects are `technically' also FAIR, but not fully open access and not reusable without restrictions.
    Level 4) The metadata as well as the data elements themselves are fully FAIR and completely public, under well defined license.
%\end{itemize}
% I don't see the points of the following sentences. Commented out for now. By Liao.
%Although the Lorentz workshop influenced and contributed significantly to the contents of the FAIR principles, the FAIR principles do not include the "levels of FAIRness" and define a metric to measure the data FAIRness. 
%Several key points in the 4-level of data FAIRness can still be seen in the FAIR principles and the sub-principles.

% This sentence is not well connected to the paragraph
%The aspirational FAIR principles lack the detailed implementation guidelines to direct the research communities to go FAIR.  

\end{comment}
The FAIR data maturity model released by the Research Data Alliance (RDA)\cite{rda2020fair} defines three elements in an evaluation framework: 1) FAIRness indicators derived from the FAIR principles to formulate measurable aspects of each principle; 2) priorities reflecting the relative importance of the indicators; and 3) the evaluation method defining a quantitative approach to report the evaluation results.
Currently, three major types of FAIRness evaluation are available to various research communities: %\cite{de_miranda_azevedo_considerations_2020}. % among all FAIRness evaluation strategies:
\begin{enumerate}[leftmargin=*]

\item{\textit{Discrete-answer questionnaire-based evaluation}}: This approach provides a checklist of single-selection questions 
%    \todo{How are the questions related to the four levels you just mentioned above?} 
to reflect the FAIR principles and related concepts. 
    It is usually accompanied by a scoring system to evaluate the FAIRness.  It requires little knowledge about the FAIR principles and is relatively straightforward to exploit the evaluation with discrete-answer questionnaire.  
    %The set of answers is tied to the FAIR principles only and not extensible to include other information.  
    %The evaluation results can be biased according to the provided answers. 
    An example question reflecting the 'F1' FAIR principle would ask if the data has persistent identification (PID), metadata and documentation describing the data.
    A zero point score can be given if no PID, metadata and/or documentation is available.  Whereas a non-zero score can be assigned for other possible answers. 
    An example of the discrete-answer evaluation is the FAIRness evaluation tool provided from RDA FAIR data maturity model. 
    %A 0 point score is given if the submitter chooses ``Level 0: No PID, no metadata and/or documentation"; or a 5 point score is given for another option ``Level 5: (Meta)data are registered or indexed in a searchable resource".
    
    \item{\textit{Open-answer questionnaire-based evaluation}:} %~\cite{wilkinson2018design,clarke2019fairshake}: 
    This approach also exploits a list of metrics reflecting the FAIR principles. 
    %Evaluation is like answering the questions from the discrete-answer questionnaire-based evaluation.
    Different from the discrete-answer approach, the open-answer approach requires concrete answers and statements to the metric as evidences to the implementation of FAIRness.  
    An example metric to the 'F1' FAIR principle is: Whether the Globally Unique Identifier (GUID) matches a GUID scheme recognized as being globally unique in a global public registry.  The evaluation expects a valid GUID submitted as an answer. 
    The open-answer approach allows the scientific communities to extend the evaluation by creating additional metrics. However, it shares the  disadvantages as the discrete-answer approach that the manual process to input answers is required and the possible biased results. 
    
    %\todo{How is the later RDF-indicator based manual evaluation fit into this big picture? Is it discrete or open question based?   Please explicitly mention/cite the manual approach and put it into the right category here, if applicable}
    
    \item{\textit{Automated evaluation}}: This approach automatically retrieves and evaluates a given digital resource, simplifies the evaluation process and eliminates the human bias. % coming from the input answers. %often indicated by a GUID. 
    %Only essential input, GUID and description of the evaluation, are required to be entered into the evaluation service/tool. 
    Automated evaluation service could also provide evaluation feedback and recommendation to improvement. 
    However, the evaluation capability of this approach is limited by the metrics chosen, the software support, target granularity of data objects, and the resource availability of the metadata providers.  For example,
    two evaluation tools,
    F-UJI\footnote{https://www.f-uji.net/index.php} 
    and FAIR-checker\footnote{https://fair-
checker.france-bioinformatique.fr/base metrics}, use different number of metrics to evaluation the license information for 'R' FAIR principle.
     Existing automated FAIR assessment services only inspect the metadata information at a coarse granularity. They check the descriptive metadata for the whole dataset and inspect the format of the dataset but do not inspect the FAIRness of data elements, the contents of the dataset.  

% moved to methodology    \todo{We should a one or two sentences to summarize the limitations of existing evaluation approaches. Then the paper naturally transitions to our methodology}
\end{enumerate}


%\subsection{FAIRification Processes (0.75 page)}
\noindent\textbf{FAIRification Processes:}
As the FAIR Guiding Principles get higher attention in various research communities, many initiatives started to advocate the application of FAIR data principles.  GO FAIR\cite{GOFAIR}, a global, stakeholder-driven and self-governed initiative, has been working towards implementations of the FAIR Guiding Principles and proposes FAIRification framework with three focuses: 
First, the formation of machine-actionable metadata; Second, the collection of machine-actionable FAIR implementation profiles (FIPs); And last, a global FAIR data service.
\begin{comment}
\begin{enumerate}[leftmargin=*]
    \item Metadata for Machines: the formulation of machine-actionable metadata components from many domain-relevant metadata requirements and policy considerations.
    \item FAIR Implementation Profile (FIP):  a collection of machine-actionable FAIR implementation choices made by a community of practice for each of the FAIR Guiding Principles. Ready-made and well-tested FIPs created by trusted communities can be reused among other communities,
    \item Global FAIR Data Services: a metadata repository that provides access to metadata in a manner that follows the FAIR Guiding Principles, e.g. the FAIR Data point\footnote{https://www.fairdatapoint.org/}.
\end{enumerate}
\end{comment}
%\todo{We need to make sure we address the three-point focuses explicitly. }
This framework  is designed to serve as the “how to” guidance to stakeholders seeking to go FAIR. 
It exploits a bottom-up approach to start with metadata preparations for datasets from various communities.  The collection of FIPs enlarges the metadata coverage to be shared among communities. 
Ultimately, a global FAIR data service stores and hosts information about datasets to provide data Accessibility, Findability and Reusability.

\begin{comment}
\begin{enumerate}
    \item Metadata for Machines Workshops: The FAIRification starts with the formulation of machine-actionable metadata components from many domain-relevant metadata requirements and policy considerations.  The goal of of Metadata for Machines workshops is to make routine use of machine-actionable metadata in a broad range of fields.
    \item FAIR Implementation Profile: The GO FAIR community has launched the development of machine-actionable FAIR Implementation Profiles (FIP), a collection of FAIR implementation choices made by a community of practice for each of the FAIR Principles. FIP representing the implementation strategies of various communities can be used as the basis to optimize the reuse of existing FAIR-enabling resources and interoperation within and between domains.
    \item FAIR Data Point: FAIR Data Point (FDP) is a metadata repository, inspired by IBM's Linked Data Platform, that provides access to metadata in a manner that follows the FAIR principles.
\end{enumerate}
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!htbp]
%\vspace{-0.15in}
 \centering
 %\vspace{-0.05in}
 \includegraphics[width =1.0\textwidth]{./figures/FAIRification.pdf}
 %\vspace{-0.2in}
 \caption{\textmd{FAIRification Process proposed by GO FAIR initiative.}}
 \label{fig:FAIRification}
%\vspace{-0.15in} 
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



Together with the FAIRification framework, the GO FAIR initiative also provides a FAIRification process aiming at addressing the conversion of raw datasets into FAIR datasets. 
These 7 steps and the the workflow are presented in Figure~\ref{fig:FAIRification}. % No space for the figure
This FAIRification process emphasizes on FAIRification for both data and metadata, including seven steps: (1) retrieve non-FAIR data, (2) analyze the retrieved data, (3) define the semantic model, (4) make data linkable, (5) assign license, (6) define metadata for the dataset, and (7) deploy/publish FAIR data resource. 
%\todo{This process seems to be important. We should have a  figure for it.}
%\todo{The figure looks nice. But some keywords may need a bit explanation, such as making data linkable. }
The process is proposed for general purpose without considering specific requirements and needs from individual community.  
Challenges may arise when applying the process for data coming from a specific domain.
For instance, without standardized data format in HPC community, the analyses used for the retrieved data vary based on the selected custom data formats.
The development of a HPC semantic model needs iterative reviews and revisions to ensure consistency in providing accurate and unambiguous meaning of entities and relations
%make it
%the semantic model
%represent a %consensus
%consistent view 
in the HPC domain.
%\todo{Any challenges we faced in our case study? Make sure we list them explicitly}

%\todo{To Pei-Hung: There are quite a few terms floating around: data object, metadata, data elements, semantic model, linkable etc. We should have a clear definition of them, with concrete examples, possibly summarized into a table.}

==> TEML'22 FAIRness-Extended-arXiv/HPCOntology.tex <==
     An  ontology is a formal specification for explicitly representing knowledge about types,  properties, and interrelationships of the  entities in a domain. 
     An ontology can provide the much needed controlled vocabularies, knowledge representation, and standards to fulfill Interoperability ("I") and  Reusability ("R")  of  the  FAIR data principles.   
     
     We have developed the HPC ontology to cover HPC specific properties including software, hardware, and their interactions.  
     The coverage of HPC ontology is expected to expand gradually as more data and information are explored.
     HPC ontology is represented with JSON-LD, a method of encoding linked data using JSON format,  for expressing data in the Resource Description Framework (RDF) data model.
     HPC ontology is described in Terse RDF Triple Language, or Turtle, for expressing data in the Resource Description Framework (RDF) data model.
     A two-level design is adopted for HPC ontology to effectively cover both high-level concepts needed in the HPC domain and more specific low-level details in subdomains. 
     The high-level components  of the HPC ontology aim to  provide descriptive,  administrative  and  statistical metadata  for  users  to annotate  datasets. 
     The top level concept, \texttt{hpc:Thing}, in the HPC ontology describes a set of fundamental properties including its unified resource identifier, the type of the ID , name, url, etc. 
     All other high-level concepts are directly or indirectly subclasses of \texttt{hpc:Thing}. Each concept inherits the fundamental properties from its superclass and also includes additional properties as needed.
     
     On the other hand, the set of  the low-level components provides concepts and relationships details for smaller domains and aims to be extensible for support rapid changes in HPC software and hardware.
     They are essential in HPC ontology by providing rich attributes to describe data elements to achieve maximal FAIRness.
     The low-level components in HPC ontology will relevant scopes in HPC including hardware, software, performance data, and AI models.
     Table~\ref{tab:xplacer-properties} list examples of properties defined in HPC ontology and needed by the Xplacer dataset.

\begin{table*}[!htp]\centering
\caption{Examples of HPC Ontology properties to annotate Xplacer dataset}
\label{tab:xplacer-properties}
\scriptsize
\begin{tabular}{|l|l|l|}\hline
\textbf{Property} &\textbf{Data type} &\textbf{Description} \\\hline
hpc:benchmark & xsd:anyURI & Link to the associated benchmark software ID in ontology\\
hpc:kenelName & xsd:string & Kernel name\\
hpc:gpuThreadBlockSize & xsd:integer & Launch block size \\
hpc:registersPerThread & xsd:integer & Register usage per thread \\
hpc:gpuThreadCount & xsd:integer & Threads count in launched kernel \\
hpc:gpuWavesPerSM & xsd:integer & Wave count in SM \\
hpc:maxGPUThreadBlockSizeLimitedByRegister & xsd:integer & Max block limited by registers \\
hpc:maxGPUThreadBlockSizeLimitedByWarps & xsd:integer & Max block limited by warps \\
hpc:cpuPageFault & xsd:integer &  CPU page fault count\\
hpc:gpuPageFault & xsd:integer &  GPU page fault count\\
hpc:hostToDeviceTransferSize & qudt:QuantityValue & Host to Device data transfer size \\
hpc:deviceToHostTransferSize & qudt:QuantityValue & Device to Host data transfer size\\

\hline
\end{tabular}
\end{table*}

==> TEML'22 FAIRness-Extended-arXiv/Xplacer.tex <==
In this paper, we pick a dataset and ML model generated by the XPlacer~\cite{xu2019machine} to study how to FAIRify HPC datasets and ML models. 
The reason to choose XPlacer is that the authors released raw data with detailed documents explaining how data was generated and processed. 
They also describe the meanings of each row and column for the corresponding CSV files.
%They also explain what each row and column means for the corresponding CSV files. 
The rich human-readable documentation provides a good foundation for FAIRness evaluation and improvement. 

XPlacer is a memory optimization tool developed to use machine learning to guide the optimal use of memory APIs available on Nvidia GPUs. 
Programmers for GPUs traditionally use a set of APIs to explicitly move data between CPU and GPU memory. 
Unified memory (UM), introduced in modern Nvidia GPU systems, greatly reduces GPU programming burdens by providing hardware-managed data migration.
A set of memory advisory APIs is also provided by Nvidia to advise the UM driver to improve performance. 
The motivation is that Nvidia provides a rich set of memory APIs and corresponding parameters. It is challenging for programmers to manually decide which API to use and with what parameter values. XPlacer aims to build machine learning models to automatically make such decisions for a program running on heterogeneous CPU/GPU machines.
It has both offline training and online adaptation steps, including collecting training datasets, generating machine learning models, and applying the generated model to predict the best memory usage advise. 


%This section presents the XPlacer background, data collection process, and AI models used in the experiments.


The offline data collection uses seven benchmarks from the Rodinia benchmark~\cite{che2009rodinia} with seven available memory advises applied  to different arrays in the benchmarks.
In each experiment with a selected benchmark, profiling tools were used to collect kernel level and data object level metrics.
%A total of 59 metrics can be gathered for each benchmark in the metric collection.
A feature correlation algorithm is applied to down select the 10 most relevant features from the original 59 metrics gathered in the metric collection.
After data normalization and feature dimensionality reduction, the collected XPlacer dataset has a total of 2688 samples prepared for the machine learning models.

\begin{comment}
\subsection{The XPlacer Project}
%\todo{Cut text+ figure to at most 1 page, rephrase it also}
Programmers for GPUs traditionally use a set of APIs to explicitly move data between CPU and GPU memory. 
Unified memory (UM), introduced in modern Nvidia GPU systems, greatly reduces GPU programming burdens by providing hardware-managed data migration.
A set of memory advisory APIs is also provided by Nvidia to advise the UM driver about the usage hints of data objects in the applications in order to improve performance. 
%These hints (such as ReadMostly, PreferredLocation, AccessedBy)
However, it is challenging for programmers to manage and assign different APIs for various data objects (e.g. arrays) used in an application.


Xplacer, an memory advice controller, was developed to guide the optimal use of mixed non-UM and UM APIs by recommending the most suitable memory advises for major arrays in a program for better performance.
It has both offline training and online adaptation 
%(shown in Figure~\ref{fig:online}) 
to collect training dataset, generate machine learning models, and apply the generated model to predict the best memory usage advise.  
%The collected datasets and machine learning models used by Xplacer are chosen in this work as the example to study the  FAIRification process for HPC datsets and AI models.  This rest of this section will covers the major components and workflow used in XPlacer.

%\subsubsection{Offline training}
%Profiler-generated metrics are used in offline phase to train a machine learning model, which subsequently is used to predict optimal memory use advice and applies this advice to applications at runtime.  


 % sorry we have to comment out this figure to save space for the key points of this paper, Liao
\begin{figure}[t]
%\vspace{-0.15in}
 \centering
 %\vspace{-0.05in}
 \includegraphics[scale=0.7]{./figures/XPlacer_workflow.pdf}
 %\vspace{-0.2in}
 \caption{\textmd{The workflow of the \texttt{XPlacer}.}}
 \label{fig:online}
%\vspace{-0.15in} 
\end{figure}

The goal of Xplacer is to predict best choice among the following different memory APIs available in CUDA~\cite{cuda_mem}:
\begin{itemize}
\item \texttt{Non-UM}: Using non-unified memory to manage a data object. This means data is explicitly copied between CPUs and GPUs.
\item \texttt{UM:Default}: Using unified memory to manage a data object, the default behavior performs on-demand page migration when no advise is specified.
\item \texttt{UM:cudaMemAdviseSetReadMostly}: With UM managing a data object, the data object is given this advise that it mostly going to be read from and only occasionally written to.
\item \texttt{UM-cudaMemAdviseSetPreferredLocation}: 
The data given this advice is set to have the preferred memory location on the device's memory or the host memory. This option has two variants: one set the preferrence location to be CPU and the other be GPU. 
\item \texttt{UM:cudaMemAdviseSetAccessedBy}: This advice implies that the data will be accessed by a specified device. Again this option has two variants: for CPU or GPU. 
\end{itemize}
As a result, a total of seven options can be given to a training sample to generate different code variants: %\texttt{DiscreteMemMalloc}, \texttt{UnifiedMemoryMalloc} default, \texttt{ReadMostly}, \texttt{PreferredLocation} for GPU, \texttt{PreferredLocation} for CPU, \texttt{AccessedBy} for GPU, and \texttt{AccessedBy} for CPU. 
The online adaptation of Xplacer will then use the trained model to find best option for new applications. More technical details of XPlacer can be find in ~\cite{xu2019machine}. 
\end{comment}


\begin{comment}

\begin{table}[t]
\small
\centering
\caption{Benchmarks with various inputs for experiments}
\vspace{0.05in}
\begin{tabular}{|l|c|c|l| c |}  \hline
    & \textbf{Kernels} & \textbf{Arrays} & \textbf{Variants} & \textbf{Inputs}   % \textbf{Mode} 
    \\  \hline
CFD  & 4 & 3 & (7$\times$7$\times$7) &  3 \\ \hline
BFS  & 2  & 4  & (7$\times$7$\times$7$\times$7) & 3  \\ \hline
Gaussian  & 2 & 3 & (7$\times$7$\times$7) &  75 \\ \hline
HotSpot  & 1 & 2 & (7$\times$7) & 8  \\ \hline
NW & 2 & 2 & (7$\times$7)  &  64 \\ \hline
LUD  & 3 & 1 & (7)  & 64  \\ \hline
PathFinder  & 1 & 1 & (7)  & 25  \\ \hline
\end{tabular}
\label{tab:benchmarks}
\end{table}
\end{comment}

%The offline metrics collection is executed with a series of experiments.
%Experiments are conducted using seven benchmarks from the Rodinia benchmark~\cite{che2009rodinia} with various memory advises applied to different arrays in the benchmark and different input options.

%\subsection{AI Models}
%TODO: introduce various models generated by Xplacer: talk to Murali if needed
%Here we present details of the machine learning model built for this task. 

%The input dataset to the machine learning model is composed of feature vectors created from the XPlacer dataset after performing necessary data normalization and feature dimensionality reduction. 
%The  training dataset sample size is 2688. 
%The output is the class of memory placement advice determined from the seven memory advice options. 

%To guarantee the robustness of Xplacer model, the 10-fold cross validation is used to verify the model's performance and also ensure the model performs evaluation on unseen data. It is to be noted that the model training phase is done only once offline. The prediction accuracy of the model is chosen as the metric of evaluation. Based on this metric, we observe that the decision tree classifier yielded highest prediction accuracy and we chose that model. 

%The training dataset obtained from the offline processing was normalized and evaluated with selected machine learning classification algorithms.
%These models that were evaluated are Decision tree using J48 algorithm~\cite{quinlan1996bagging}, Random Forest~\cite{breiman2001random}, Bagging algorithms~\cite{quinlan1996bagging}, RandomTree~\cite{randomtree} and REPTree \cite{randomtree}. 
%To guarantee the robustness of our model and avoid overfitting, we use the 10-fold cross validation method to measure the prediction accuracy. Thus, we ensure the model's performance is measured based on its predictions on unseen data. We rely on the model's prediction accuracy as the metric of evaluation since the GPU memory choice determined by this model has a direct correlation to the program execution time. 

\begin{comment}

\subsubsection{Online adaptation}
The online adaptation first collects and normalizes the runtime metrics from the target application that runs in default mode using discrete memory (step 1 in Figure~\ref{fig:online}). 
The generated classifier model is then called at runtime to predict and set the best memory usage advice option value for each of the instances (step 2 and 3 in Figure~\ref{fig:online}). %(i.e., the data object in the given application).
An instance represents a kernel's execution using a specific input data, with memory advise given to data objects used in the given kernel.
Finally, \texttt{XPlacer} automatically executes the staged input source code to enable the execution using the selected memory advice choices (step 4 and 5 in Figure~\ref{fig:online}).


%The first two phases contribute most of the data creation and processing for the machine learning model creation.  This paper will focus on the data collection and feature engineering phases to evaluate the FAIRness of the data used in the Xplacer.
\todo{Fig 2. can be removed. Section III only needs 1 page to describe rough idea and majority is about the data.}
\end{comment}

\begin{comment}
\subsection{Datasets}

The offline data collection uses seven benchmarks from the Rodinia benchmark~\cite{che2009rodinia} with seven available memory advises applied  to different arrays in the benchmarks.
%Table~\ref{tab:benchmarks} summarizes the information of the selected benchmarks and the total available variants for each benchmark. 
In each experiment with a selected benchmark, two Nvidia profiling tools,  Nsight and NVprof, were used to collect kernel level and data object level metrics respectively.
A total of 59 metrics can be gathered for each benchmark in the metric collection.
A feature correlation algorithm is then applied to down select the 10 most relevant features. 
%from the dataset by evaluating the worth of a feature by measuring the Pearson's correlation between the feature and its class.
%\begin{comment}
The final selected features for the model training are: block size,
registers per thread,
number of threads,
waves per SM,
block limit registers,
block limit warps,
CPU page faults,
GPU page faults,
HtoD memory transfers, and
DtoH memory transfers.
%\end{comment}
After data normalization and feature dimensionality reduction, the collected Xplacer dataset has a total of 2688 samples prepared for the machine learning models.
\end{comment}


%\todo{a figure showing data processing pipeline: and which data in the pipeline is made available. Looks like the final labeled dataset is the focus of this paper } \Hailu{add the figure here: Fig 3}


The raw data collected from XPlacer experiments is hosted at a public Github repository\footnote{https://github.com/AndrewXu22/optimal\_unified\_memory}. Figure~\ref{fig:csv} shows how the raw profiling data generated from different GPU machines are first parsed and stored into CSV files, which are merged and labeled to generate training datasets to build various machine learning models.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!ht]
%\vspace{-0.15in}
 \centering
 %\vspace{-0.05in}
 \includegraphics[scale=0.45]{./figures/csv.pdf}
 %\vspace{-0.2in}
 \caption{\textmd{XPlacer data processing pipeline}}
 \label{fig:csv}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{comment}
Contents stored at the repository includes: 
\begin{itemize}
    \item Source codes of benchmarks, data processing scripts and the auxiliary files used in the data collection.
    \item CSV files (e.g. ./kernel-level-measurement/dataset.csv) storing GPU kernel-level metrics for each benchmark measured by the profiling tools.The files include columns indicating kernel names, input data size,  GPU memory utilization rates, execution duration, thread block size, and so on.
    \item CSV files (e.g. ./data-level-measurement/GPUTrace.csv) storing GPU data-object-level metrics for each benchmark measured by the profiling tools.  The files include columns for array names (data objects) and information related to array's begin memory address, end memory address, CPU page faults, GPU page faults, Host-to-Device data transferring size, Device-to-Host data transferring size and so on. 
    \item CSV files (e.g. mergedDataSet.csv) including jointed dataset merged from the kernel-level and data-object-level. 
    \item CSV files (e.g. labelledData.csv) with labels to identify the best-performing variant for a kernel from a benchmark with a specific input. 
    \item Attribute-Relation File Format (ARFF) files storing transformed contents from the labelled CSV files using Weka\cite{hall2009weka}.  %\todo{What transformations are used here? feature correlation to reduce dimensionality??} 
% The input CSV file for the conversion to ARFF file is a CSV file that collects all the labelled data processed for for all benchmarks.
\end{itemize}
\end{comment}

The readme.md of the git repo has detailed information for all released files, especially what each column means for the release CSV files. Table~\ref{tab:csv-kernel-data}, \ref{tab:csv-profiling} and \ref{tab:csv-gpu} show the labelled CSV files' columns in different sections, including those for kernels and data objects, profiling metrics, and GPU properties.  The Code variant ID column is used to represent an memory advise given to data objects in a kernel. 
%This gives us a good start point to make datasets FAIR.
\begin{table}[!htp]\centering
\caption{CSV columns for kernels and data objects}\label{tab:csv-kernel-data}
\scriptsize
\begin{tabular}{|l|l|}\toprule
\textbf{Column Name} &\textbf{Description} \\\midrule
Benchmark & Benchmark software name \\
commandLineOption& Representing data size or input files etc. \\
KernelName &GPU kernel name \\
ArrayName (Data) &Name of the array \\
ArrayID (ID) &Internal integer ID of the array \\
Variant & Code variant ID  \\
labeledVariant (label) &The best performing code variant ID \\
AllocatedDataSize (DataSize) &Memory allocation size \\
BeginAddr &Beginning address of memory allocation \\
EndAddr &Ending address of memory allocation \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!htp]\centering
\caption{CSV columns for profiling metrics}\label{tab:csv-profiling}
\scriptsize
\begin{tabular}{|l|l|}\toprule
\textbf{Column Name} &\textbf{Description} \\\midrule
Elapsed Cycles & Cycle count of profiled code \\
TotalExecutionTime &Total execution time for this kernel.e.g \\
NumberOfCalls &Number of calls to this kernel \\
AverageExecutionTime &Average kernel execution time(ms) \\
MinExectionTime &Minimal kernel execution time \\
MaxExecutionTime &Maximal kernel execution time \\
ExecutionTimePercentage &Percentage of time spent in this kernel (\%) \\
MemoryThroughputPercentage &GPU memory throughput \\ %w.r.t. theoretical peak (\%) \\
SOL DRAM & DRAM utilization \\ %w.r.t. the theoretical maximum \\
SM [\%] &SM throughput \\ %w.r.t. theoretical peak (\%) \\
SOL L1/TEX Cache & L1/Tex cache utilization \\ %w.r.t. the theoretical maximum \\
SOL L2 Cache & L2 cache utilization \\ %w.r.t. the theoretical maximum \\
Achieved Occupancy &Achieved profiled occupancy \\
Achieved Active Warps Per SM &Profiled active warps per SM \\
CPUPageFault &CPU page fault count \\
GPUPagePault &GPU page fault count \\
HtoD &Host to Device transfer size \\
DtoH &Device to Host transfer size \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!htp]\centering
\caption{CSV columns for GPU properties}\label{tab:csv-gpu}
\scriptsize
\begin{tabular}{|l|l|}\toprule
\textbf{Column Name} &\textbf{Description} \\\midrule
DRAM Frequency &Frequency of DRAM \\
SM Frequency &Frequency of Streaming multiprocessor \\
SM Active Cycles &Active cycle counts from SM \\
Theoretical Active Warps per SM &Theoretical Active Warps per SM \\
Theoretical Occupancy &Theoretical Occupancy \\
Block Limit SM &Max block limited by SM \\
Block Limit Registers &Max block limited by registers \\
Block Limit Shared Mem &Max block limited by shared memory \\
Block Limit Warps &Max block limited by warps \\ \midrule
\multicolumn{2}{|c|}{GPU Configuration Information}\\ \midrule
Block Size &Launch block size \\
Grid Size &Launch grid size \\
Registers Per Thread &Launch register//thread \\
Shared Memory Configuration Size &Launch shared memory configuration size \\
%Driver Shared Memory Per Block & \\
%Dynamic Shared Memory Per Block & \\
Static Shared Memory Per Block &Launch static shared memory \\
Threads &GPU thread count \\
Waves Per SM &Launch wave per SM \\
RemoteMap &Unified memory remote map \\
\bottomrule
\end{tabular}
\end{table}



Multiple machine learning classification models were generated by XPlacer from the training datasets. These models include Random Forest, Random Tree and Decision Tree. Figure~\ref{fig:decision_tree} shows a partial view of the decision tree model in XPlacer. 
Each tree node in the decision tree represents a decision determined by a feature with a threshold value. 
When the value of the feature is less and equal than the threshold value, the decision tree will move downward to the left node of the tree.
Otherwise, it moves downward to the right child node.
%For example, the decision at the root node in Figure~\ref{fig:decision_tree} compares the value of feature "Executed Ipc Elapsed" and the threshold value $0$.  When the Ipc Elapsed value is less and equal to 0, the decision moves into its left child and continues to check the next feature "GPU page fault" and an associated threshold value $0.00743$.
The tree traversal continues to move downward and compare various features and threshold values until it reach to a tree leaf node which represents a label value.  A label value represents the final decision made by the decision tree model.  
For Xplacer, the label value represents the memory advise that will be recommended by the machine learning model. 

\begin{comment}
We explicit the details of decision tree model by following the left subtree. Among this partial tree, the root node starts with the value of Executed Ipc Elapsed, using a threshold value of 0. This results in two nodes. When the value of Executed Ipc Elapsed is less than or equal to 0, at the left node of the second layer, the value of GPU Page Fault will be evaluated by a threshold of 0.000743. At this time, when the value of GPU Page Fault is greater than 0.000743, then the model will decide a label 0 to the given data instance. Otherwise, it will go to the left node at the third layer with the value of Waves Per SM. At this node, if the value of Waves Per SM is greater than 0, the model will decide the label 1 to the data instance. Otherwise, it will go to the left child node and evaluate the value of GPU Page Fault. At this layer, with the threshold of 0.000149, the model can decide either label 0 or 4 for the data instance. Figure~\ref{fig:decision_tree} displays a small portion of the overall tree model, in XPlacer, the overall decision tree model will evaluate the data instances by using all 10 features in the dataset.
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!htbp]
%\vspace{-0.15in}
 \centering
 %\vspace{-0.05in}
 \includegraphics[scale=0.25]{./figures/decision_tree.pdf}
 %\vspace{-0.2in}
 \caption{\textmd{A partial view of the decision tree model of XPlacer.}}
 \label{fig:decision_tree}
%\vspace{-0.15in} 
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[t]
%% %\vspace{-0.15in}
%  \centering
%%  %\vspace{-0.05in}
%  \includegraphics[scale=0.49]{./figures/Xplacer-decision-tree.pdf}
%%  %\vspace{-0.2in}
%  \caption{\textmd{A partial view of the decision tree that shows the feature branches through the %data placement choices.}}
%  %(underlined and enumerated from Table \ref{gaussian-variant}).}}
%  \label{fig:decisiontree}
%% %\vspace{-0.15in} 
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%

==> TEML'22 FAIRness-Extended-arXiv/conclusion.tex <==
\noindent\textbf{Summary:}
 This paper presents a concrete methodology and a case study to make HPC datasets and ML models FAIR, after surveying existing techniques used to assess and improve FAIRness of scientific data. 
Our methodology can enjoy the benefits of both automatic and manual assessments while avoiding their limitations. 
It also includes a set of actionable suggestions to address reported FAIRness issues, including using ontologies to provide rich and standard data attributes. 
The experiment has shown that our methodology can effectively improve the FAIRness maturity for a selected dataset and ML model.    

\noindent\textbf{Discussion:}
To make general datasets and ML models FAIR, it can be discussed from three different aspects:
\begin{itemize}[leftmargin=*]
    \item FAIRness assessment: In this study, we have observed that existing FAIRness assessment tools have several major weaknesses:  insufficient coverage for details in FAIR principles, tendency to report biased assessment result, with emphasis to limited group of users (data curators, data stewards, and data users), and with support for only specific domains (with  attributes and vocabularies in specific scientific communities).  
    Improving the FAIRness assessment support addressing the above weaknesses can provide a trustworthy gauge of data FAIRness.  Data generators, curators, stewards and users can jointly improve the data FAIRness based on a standardized and creditable metric of data FAIRness. 
    \item FAIR-aware data store and management: Data hosting and management service have great impact to the FAIRness for the hosted/managed data. In this paper, \texttt{zenodo.org} is recommended for its support in DOI generation, general metadata, provenance and license information support.  It provides relatively smooth transition for users, who heavily rely on git repositories to store data and digital contents, to FAIRify the data.
    Several leading services for hosting/managing ML datasets and models \cite{huggingface,kaggle,hosny2019modelhub,openml} are commonly used by ML developers and users. 
    We survey and evaluate their support for FAIRness and observe several commonly seen issues: missing persistent identifier representing the datasets or models, insufficient coarse and fine-level metadata, 
    and accessing (meta)data and model is constrained by hosting service APIs.
    Providing FAIR-aware data store and management systems is also a critical factor to make general datasets and ML models FAIR. 
    \item FAIRification for ML models: As FAIR principles are applicable to any digital object, FAIRness for ML models should also be considered.
    We apply data annotation with support from HPC Ontology as an example to achieve FAIRness fulfilment for the selected decision tree model.
    However, the same approach might not be practical to many large scale ML models that contain millions or billions of parameters.
    Supporting rich metadata describing the ML models would be the alternative approach for the FAIRification.
    There is not yet a dedicated list of attributes and metadata information to represent all ML models (reflecting 'R1' sub-principle). 
    We also observe there are many information associated with the Interoperability and Reusability of a ML model cannot easily be found.
    For example, the NLP model BERT comes in many flavors: varying its size, preprocessing applied to the dataset (case and special characters), and additional fine-tuning objectives.
    Such information might not be shown by existing model hosting services and cannot be checked by any FAIRness assessment tool. 
    And last, ML models closely related to the datasets used for training.  The reusability of a ML model is likely to be limited to a specific type of dataset, or learning goal.
    Attributes describing the dataset requirements and learning goal need to be properly defined.
    Therefore, identifying the FAIR-centric metadata and attributes for the ML models (e.g.\ model architecture, training configuration, and training objectives), together with automated evaluation to assess the metadata, can greatly promote the FAIR for ML models.  
%    Based on our survey, a list of  attributes are candidates: model architecture details, type of tasks, training configuration, dataset preparation details.
    
\end{itemize}

%For the unfulfilled FAIRness maturity indicators, implementations are in the development roadmap to improve the FAIRness maturity. We expect that HPC ontology can be adopted as the standard to define data and metadata within the HPC community.

%The FAIR Guiding Principles suggest guidelines in data preparation to make data findable, accessable, interoperatable and reusable.
 %Key attributes of FAIR data includes persistent identifiers, rich and comprehensive metadata describing the data, structured and machine-actionable data format, links among public shared data and metadata, license and data provenance information specified.   
% The case study with XPlacer dataset represents one type of HPC research workflow that has collected data represented in the tabular CSV format.  
% The limited metadata support in such tabular format leads to low fulfilment in data FAIRness.
% A HPC ontology, proposed and implemented in this work, aims to provide rich and complete metadata information for HPC datasets and help to improve the data FAIRness.
%The highest FAIRness for XPlacer dataset is achievable following the suggested tasks.
\noindent\textbf{Future work:}
We will continue to improve the HPC ontology to have required references to other data standards.  We hope that the HPC ontology can be adopted as one standard to FAIRify data within the HPC community. 
We will also incorporate some manual correction and assessment steps into the automated assessment step to further improve the FAIRness assessment. 
Last but not the least, we will extend our work to support FAIRification for ML models and workflows.  
Ultimately, we aim to pursue trustable machine learning by achieving better FAIRness in machine learning models and datasets.
%To fully utilize the structured and linked data from HPC ontology, and how to synthesize HPC datasets through the ontology queries to enable machine learning workflow is part of %placed in 
%the future research plan.


==> TEML'22 FAIRness-Extended-arXiv/discussion.tex <==
This section presents the FAIRification process of applying our methodology, presented in section~\ref{Fairify}, to the XPlacer datasets and the decision tree model. 
%Due to page limit, we only elaborate the work on the datasets since the work for the AI models is very similar. 

%\subsection{Initial Assessment}
\noindent\textbf{Initial Assessment:}
The initial hybrid assessment results shown in Figure~\ref{fig:initEval}  reveal that a selected XPlacer dataset (generated on an IBM machine) has a 19.1\% FAIRness score. 
%\todo{I cannot parse this portion. Please rephrase it: 9 out of maximum 47 full score value and a highest fulfillment in `A' FAIR principle (46.2\%)}. 
%The score from F-UJI automated assessment shows 14\% fulfillment as a result (3.5 out of maximum 24 fulll score value).
The visual reports from the RDA manual evaluation and the detailed report from the F-UJI evaluation reveal that persistent identifier is missing to fulfill the `F' FAIR principle.  
Missing license and provenance information are the major factors for its low fulfillment in the `R' FAIR principle.  
For the rest covered in `A' and `I' FAIR principles,
missing metadata information is the root cause for its low fulfillment in FAIRness.  
 \begin{comment} % very confusing content. 
 It is worth noting that the score values represent only relative information for the evaluation.\todo{relative to what? previous datasets evaluated by the website? This info. should be introduced when we first mention the scores generated by the website.  What scores do we use as the final verdict? Do we use relative or absolute metrics? This is very important.}
A higher fulfillment simply implies a relatively higher readiness for data FAIRness is achieved.
Among all the metrics with 0 point obtained, FsF-F1-02D is about the persistent identifier for the dataset and FsF-R1.3-02D is about the file format for the data contents.  The rest are all related to missing or insufficient metadata information.  
This initial assessment concludes that Xplacer misses persistent identifier, license information, and has weak metadata support to fulfill FAIR principles.  
Assessment with the manual evaluation is also conducted.  The initial result shown in Fig.~\ref{fig:initEval} reflects the reality that many details in the FAIR principles were not considered when the data was released.
\end{comment}

\begin{comment}

\begin{table*}[htbp]\centering
\caption{Initial Automated FAIRness evaluation for Xplacer using F-UJI\todo{is title accurate?}}
\label{tab:initEval}
\scriptsize
\begin{tabular}{|c|c|c|p{5cm}|c|c|c|} \hline
\textbf{Metrrics}&\textbf{Max score} & \textbf{Score} & \textbf{Initial assessment explanation} & \textbf{score v.1} & \textbf{score v.2} & \textbf{score v.3}  \\ \hline
FsF-F1-01D & 1 & 1 & Unique identifier schemes found ['url'] & 1 & 1 & 1\\ \hline
FsF-F1-02D & 1 & 0 & Not a persistent identifier scheme -: url & 1 & 1 & 1\\ \hline
FsF-F2-01M & 2  & 0.5 & Metadata has been made available via common web methods
Core data citation metadata and descriptive metadata are not available & 1 & 1 & 2\\ \hline
FsF-F3-01M &1 & 0 & No metadata for data content related information and PID or URL which indicates the location of the downloadable data content & 0 & 1 & 1\\ \hline
FsF-F4-01M & 2 & 0 & Metadata cannot be retrieved by machine and is not registered in major research data registries & 2 & 2 & 2\\ \hline
FsF-A1-01M & 1 & 0 & No metadata specified for data access informatiton & 1 & 1 & 1\\ \hline
FsF-A1-02M & 1 & 1 & Standard protocol for access to metadata found -: https & 1 & 1 & 1\\ \hline
FsF-A1-03D & 1 & 0 & No metadata describing communication protocol & 0 & 1 & 1\\ \hline
FsF-A2-01M & & N/A & & N/A & N/A & N/A \\ \hline
FsF-I1-01M & 2 & 0 & No metadata using formal knowledge representation languages & 2 & 2 & 2\\ \hline
FsF-I1-02M & 1 & 0 & No semantic resource found for metadata & 0 & 0 & 0\\ \hline
FsF-I3-01M & 1 & 0 & No related resource retrieved from metadata & 1 & 1 & 1\\ \hline
FsF-R1-01MD & 4 & 0 & No metadata specifying the content of data & 1 & 1 & 1 \\ \hline
FsF-R1.1-01M & 2 & 0 & License information unavailable in metadata & 1 & 1 & 1\\ \hline
FsF-R1.2-01M & 2 & 1 & Found Github as  data creation-related provenance information, but formal provenance metadata is unavailable & 1 & 1 & 1\\ \hline
FsF-R1.3-01M & 1 & 0 & No metadata following a standard recommended by the target search community of data & 1 & 1 & 1\\ \hline
FsF-R1.3-02D & 1 & 0 & Could not perform file format checks as data content identifier(s) unavailable/inaccessible & 0 & 1 & 1 \\ \hline
\end{tabular}
\end{table*}
\end{comment}


\begin{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.35\textwidth}
         \centering
\includegraphics[scale=0.35]{./figures/Inital_Eval.png}
        \caption{Initial FAIRness score}
        \label{fig:initEvalA}
\end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.55\textwidth}
         \centering
 \includegraphics[scale=0.35]{./figures/RDA-Eval.pdf}
      \caption{Initial assessment FAIRness maturity levels}
      \label{fig:initEvalB}
     \end{subfigure}
     \hfill
        \caption{Initial hybrid assessment}
        \label{fig:initEval}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!ht]
     \centering
    \begin{minipage}{.45\linewidth}
        \begin{subfigure}[t]{.9\linewidth}
            \includegraphics[scale=0.3]{./figures/fig2_1.png}
            %\caption{Detail van een route}
            %\label{fig:weather_filter1}
        \end{subfigure} 
        \begin{subfigure}[b]{.9\linewidth}
            \includegraphics[scale=0.3]{./figures/fig2_2.png}
           \caption{Initial FAIRness score}
        \label{fig:initEvalA}
        \end{subfigure} 
        
    \end{minipage}
     \begin{minipage}{.52\linewidth}
            \begin{subfigure}[t]{.9\linewidth}
                \includegraphics[scale=0.31]{./figures/fig2_3.png}
                \caption{Initial FAIRness maturity levels}
                \label{fig:initEvalB}
            \end{subfigure}
        \end{minipage}
        \caption{Initial hybrid assessment}
        \label{fig:initEval}
        \vspace{-0.1in}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Improving FAIRness}
\noindent\textbf{Improving FAIRness:}
%To achieve highest FIARness, :
%First group of tasks address only the weakness exposed from the initial FAIRness assessment and aim to obtain the higher scores reported from the assessment service. 
%Second, we improve the dataset to aim for improve FAIRness maturity in data content granularity.
% We have no space for AI model . Performance d
%And last, we extend FAIRification support to cover AI models used by XPlacer dataset.
With the assessment feedback and recommendations, we apply the methods mentioned in Section~\ref{sec:improvingMethods} to achieve a higher assessment result.
\begin{itemize}[leftmargin=*]
\item We uploaded the XPlacer dataset to \texttt{Zenodo.org} to obtain an DOI for persistent identifier.  %The uploaded data also becomes more discoverable with Zenodo's registry service for general-purpose usage.  
With the DOI available, assessment can pass FAIR evaluation metric FsF-F1-02D.
%\todo{tentatively using https://doi.org/10.5281/zenodo.4902130 for testing, will update the final one}

\item As part of the uploading process, we carefully filled in required metadata information in Zenodo. The enhancement is able to fulfill eleven more metrics.
% comment out the list unless it's needed. (FsF-F4-01M, FsF-A1-01M, FsF-I1-01M, FsF-I3-01M, FsF-R1-01MD, FsF-R1.1-01M, FsF-R1.2-01M, and FsF-R1.3-01M)  (FsF-F3-01M, FsF-A1-03D, FsF-R1.3-02D) and FsF-F2-01M 

\item Basic provenance information is also provided by Zenodo. However, Zenodo does not provide formal provenance metadata such as PROV.  Therefore, only partial fulfillment is achieved for metric FsF-R1.2-01M.

\item We also chose the Creative Commons 4.0 license (CC-BY 4.0) for the XPlacer dataset to fulfill the R1.1 principle.

\item We extended the HPC ontology~\cite{liao2021hpc} to provide required rich attributes to describe fine-grain data elements. A special unit ontology (QUDT) is also used to annotate the units for numerical values to enable maximum data interoperability and fulfill the RDA-I3-01M FAIRness indicator. % \todo{to address what metrics??} 



\item We used Tarql to automatically convert the corresponding CSV file into linked data using the JSON-LD format, with attributes provided by the HPC Ontology. Listing~\ref{jsonoutput} shows an example output of the conversion. A set of key-value pairs are generated to describe data cells of a CSV file. Each key is a standard metadata tag or an attribute provided by an ontology. For example, \textit{hpc:hostToDeviceTransferSize} at line 9 is used to indicate CPU to GPU data transfer size. The corresponding value at line 10 is pointing to an object defined between line 13 and 23, which include two other nested objects for precisely encoding unit (KiloByte) and value (7872.0), respectively. This level of fine-grain details is required to enable maximal interoperability among datasets. 

\item For the decision tree model,
High-level metadata describing the model is provided in the FAIRification process.  
In addition,
we leverage and extend HPC ontology to provide standard attributes to annotate fine-grain information in the decision tree.
The decision tree model can then be presented as linked data using JSON-LD format tree by annotating the tree nodes with the feature and threshold value for the non-leaf nodes and the label property for the leaf nodes. 


\end{itemize}
\begin{lstlisting}[numbers=left, basicstyle=\tiny, captionpos=t, caption=Example JSON-LD output, label={jsonoutput}]
{
  "@id": "http://example.org/test.csv#L1",
  "@type": "hpc:TableRow",
  "hpc:codeVariant": "111100",
  "hpc:allocatedDataSize": 8000000,
  "hpc:arrayID": "0",
  "hpc:commandLineOption": "graph1MW.6",
  "hpc:gpuPageFault": 5,
  "hpc:hostToDeviceTransferSize": {
    "@id": "_:Nbdd222a0d12a483d8f1a4cef274f18fc"
  }
},
{
 "@id": "_:Nbdd222a0d12a483d8f1a4cef274f18fc",
  "@type": "http://qudt.org/schema/qudt/QuantityValue",
  "http://qudt.org/schema/qudt/unit": {
    "@id": "http://qudt.org/vocab/unit/KiloBYTE"
  },
  "http://qudt.org/schema/qudt/value": {
    "@type": "http://www.w3.org/2001/XMLSchema#decimal",
    "@value": "7872.0"
  }
}
\end{lstlisting}



%\subsubsection{Improvements FAIRness at finer level}

 %CSV is the data format used by Xplacer to store raw text output from the performance tools and the processed data after data labelling.  \todo{Do we focus on raw data csv or labelled CSV? }
 %The tabular structure in CSV is easy to process and human readable.  
 %However, the CSV format stores only limited meta information in the header to describe the data contents and the data/metadata is not linked to other data and metadata.  
 %It is not adequate to use CSV format alone to fully fulfill the FAIR principles.
 %Additional support is needed to provide rich metadata information for the data stored in CSV format.
 
 \begin{comment}
 
The design and implementation of HPC ontology are presented in the following sections. 
  %\begin{itemize}
     \paragraph{HPC Ontology}  
     An  ontology is a formal specification for explicitly representing knowledge about types,  properties, and interrelationships of the  entities in a domain. 
     An ontology can provide the much needed controlled vocabularies, knowledge representation, and standards to fulfill Interoperability ("I") and  Reusability ("R")  of  the  FAIR data principles.   
     
     We have developed the HPC ontology\todo{cite our ontology paper here} to cover HPC specific properties including software, hardware, and their interactions.  
     The coverage of HPC ontology is expected to expand gradually as more data and information are explored.
%     HPC ontology is represented with JSON-LD, a method of encoding linked data using JSON format,  for expressing data in the Resource Description Framework (RDF) data model.
     %HPC ontology is described in Terse RDF Triple Language, or Turtle, for expressing data in the Resource Description Framework (RDF) data model.
     A two-level design is adopted for HPC ontology to effectively cover both high-level concepts needed in the HPC domain and more specific low-level details in subdomains. 
     The high-level components  of the HPC ontology aim to  provide descriptive,  administrative  and  statistical metadata  for  users  to annotate  datasets. 
     The top level concept, \texttt{hpc:Thing}, in the HPC ontology describes a set of fundamental properties including its unified resource identifier, the type of the ID , name, url, etc. 
     All other high-level concepts are directly or indirectly subclasses of \texttt{hpc:Thing}. Each concept inherits the fundamental properties from its superclass and also includes additional properties as needed.
     
     On the other hand, the set of  the low-level components provides concepts and relationships details for smaller domains and aims to be extensible for support rapid changes in HPC software and hardware.
     They are essential in HPC ontology by providing rich attributes to describe data elements to achieve maximal FAIRness.
     The low-level components in HPC ontology will relevant scopes in HPC including hardware, software, performance data, and AI models.
     
     %The HPC ontology is linked to  existing  ontologies for two purposes.  First,  
     %Through the linking to other existing ontologies, HPC ontology can reuse contents defined in existing ontologies to cover sub-domains information.
     %It can also link  the  content  of  HPC ontology  with  equivalent concepts  and  relationships  from  mainstream  ontologies to maximize the interoperability.
     %Metadata information that is not available in any existing ontology will be defined and added into HPC ontology.
     %The HPC ontology is planned to be released to public, in a regular releasing schedule, to provide improved coverage for HPC-specific information.
     %An associated DOI will be obtained for every release version for persistent identification.
     %Once HPC ontology provides sufficient coverage, it is released publicly with a DOI for persistent identification.


\paragraph{Annotating XPlacer Dataset}
    A rich set of HPC properties and vocabularies is made available by the HPC ontology development. 
%     Metadata information in HPC ontology can be retrieved by the SPARQL, a query language for Resource Description Framework (RDF).
%  The metadata information becomes persistent and linked through the connection to HPC ontology and fulfills the findable, accessable, and interoperable principles of the FAIR principles.
%     To encode the Xplacer dataset content into HPC ontology, the data stored in CSV format needs to be converted into a data format that is suitable for RDF.
     We leverage the Tarql tool\cite{tarql} for converting CSV files to RDF by querying delimited files  using SPARQL 1.1 syntax, to accomplish the format conversion.  

     Tarql takes the CSV as input and convert it into the output format in N-Triples for expressing data in the RDF data model.
     Listing~\ref{tarql} presents code snippet from the tarql query file. 
     In the code snippet,
     prefix declarations, with keyword \texttt{PREFIX}, define abbreviating URIs for HPC ontology, RDF syntax, QUDT and XML schema.
     The CONSTRUCT query form , with keyword \texttt{CONSTRUCT}, takes each query solution in the solution sequence, substitutes for the variables in the graph template, and combines the triples into a single RDF graph by set union. A RDF graph is specified by a graph template is returned by the CONSTRUCT query.
     The input CSV file can be specified by the \texttt{FROM} clause or be given as a Tarql command line option.
     A \texttt{WHERE} clause provides the basic graph pattern to match against the data graph.
     The \texttt{BIND} form allows a value to be assigned to a variable from a basic graph pattern or property path expression.

%\todo{Again, the discussion of ontology development, how to annotate CSV with ontology should go into the methodology section. This section only show the example results using XPlacer.}
     We use \texttt{BIND} to specify the data type, defined in XML schema, of data from the CSV format and assign the data to a variable used in the RDF.
     
     
     Data in the Xplacer dataset can have associated units collected from the experiments.  
     For example, DtoH in Xplacer dataset represents the memory size copied from the device memory to the host memory.
     This type of data is handled differently in the CONSTRUCT query by explicitly specifying the RDF triple.
     We leverage the rich collection of units defined in QUDT to specify the associated units for the data.
     A RDF output, in N-Triples format, will be generated according to the queries specified in the Tarql query file.
     A second conversion, from N-Triples format to JSON-LD, is performed with features supported by RDFLib. 
     An example using a simplified input in Table~\ref{tab:csvexample} generates the corresponding JSON-LD output shown in Listing~\ref{jsonoutput}.
     A row of data in the CSV file is converted into a object with an array of elements in JSON format.
     The metadata in the JSON format can be identified by an associated URI and the value of the data is specified by the \texttt{@value} syntax.
     
     %To make the data content in CSV files fulfilling the FAIR principles, our investigation leverages the Tarql tool for converting CSV files to RDF using SPARQL.
     %Tarql requires a query file written in SPARQL to define the queries for retrieving metadata information from HPC ontology.
     %The output of Tarql is in the N-triple format and provides URIs for both data and metadata from the original CSV data.
     %After RDF conversion, both data and metadata from the original CSV format maximize the fulfillment for the FAIR principles.

\begin{lstlisting}[captionpos=t, caption=Tarql query example for HPC ontology, label={tarql}]
PREFIX hpc: <http://example.org/hpc-ontology.ttl#>
PREFIX rdf: <http://www.w3.org/1999/02/22-rdf-syntax-ns#>
PREFIX qudt: <http://qudt.org/schema/qudt/>
PREFIX xsd: <http://www.w3.org/2001/XMLSchema#>
CONSTRUCT {
  ?URI a hpc:TableRow;
  # properties for experiments
    hpc:commandLineOption ?InputDataStr;
    hpc:kernel ?KernelStr;
    hpc:Variant ?variantStr;
    hpc:gpuThreadBlockSize ?BlockSizeFP;
    hpc:GridSize ?GridSizeFP;
  # properties for hardware details
    hpc:dramFrequency ?DRAMFrequencyDec;
    hpc:streamingMultiprocessorFrequency?SMFrequencyDec;
  # properties for metrics
    hpc:Cycle ?ElapsedCyclesDec;
    hpc:memoryThroughputRate ?MemoryPercentageDec;
    hpc:deviceToHostTransferSize 
    [ rdf:type qudt:QuantityValue ; 
      qudt:value ?DtoHFP; 
      qudt:unit unit:KiloBYTE ];
    hpc:hostToDeviceTransferSize 
    [ rdf:type qudt:QuantityValue ; 
      qudt:value ?HtoDFP; 
      qudt:unit unit:KiloBYTE ];
...}
FROM <file:rodinia-nw-lassen.csv>
WHERE {
  BIND (URI(CONCAT('http://example.org/rodinia-nw-lassen.csv/', ?No)) AS ?URI)
  BIND (xsd:string(?InputData) AS ?InputDataStr)
  BIND (xsd:string(?Kernel) AS ?KernelStr)
  BIND (xsd:string(?variant) AS ?variantStr)
  BIND (xsd:decimal(?Block)Size) AS ?BlockSizeFP)
  BIND (xsd:decimal(?GridSize) AS ?GridSizeFP)  
  BIND (xsd:decimal(?Memory_Frequency) AS 
        ?DRAMFrequencyDec)
  BIND (xsd:decimal(?Elapsed_Cycles) AS 
        ?ElapsedCyclesDec)
  BIND (xsd:decimal(?Memory_\[\%\]) AS 
        ?MemoryPercentageDec)
  BIND (xsd:decimal(?DtoH) AS ?DtoHFP)
  BIND (xsd:decimal(?HtoD) AS ?HtoDFP)
...}

\end{lstlisting}

\begin{table}[!htp]\centering
\caption{Examples CSV input}
\label{tab:csvexample}
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|}\hline
DataID & variant & InputData & DataSize   & GPUPagePault & HtoD \\
\hline
  0    & 111100    & graph1MW.6 & 8000000      & 5 & 7872.0 \\
\hline
\end{tabular}
\end{table}

\end{comment}



\begin{comment}  % We have no space for MODEL FARIFICATION, maybe for a journal version in the future. 
\subsubsection{AI Models FAIRification}
\todo{Again, the generic steps of model fairification should go into the methodlogy section. The current writing is hard for readers to extract the reusable process from the XPlacer example section.}
%\subsubsection{FAIRify the AI models} 
As FAIR principles are applicable to any digital object, the FAIRness of AI models should also be considered. We proposes the AI model FAIRification process including the following steps:  
%Although we do not apply FAIR principles directly to generated AI models or the AI models from the AI toolkits, we aim to make the workflow of generating AI models FAIR.
1) Whenever possible, standardized model formats,  \texttt{ONNX} (Open Neural Network eXchange)~\cite{onnx} as example, should be used to improve the accessibility, interoperability, and reusability.  
Models prepared with \texttt{ONNX} can easily be shared and applied to major machine learning frameworks.
2) Providing metadata support for AI models. Again, we use and extend the HPC ontology to provide metadata needed. The ontology is able to describe the workflows needed to generate a AI model with the associated dataset.
A workflow, that consists of commands and scripts, can prepare the data and trigger the model generation.  
As a workflow being encoded in the HPC ontology, it can easily be queried and reused to generate the AI model.
3) encoding internal details of a given model.  Due to the diverse types of machine learning models, additional supplemental, low-level components are needed to encode different types of models. 

%An AI model serves as an interface to perform prediction tasks either classification or regression etc.  Xplacer leverages Weka \cite{hall2009weka}, a Java-based machine learning toolkit with a collection of machine learning algorithms for data mining tasks, to generate the AI model. The storage format for the model generated by Weka is proprietary \texttt{.model} format and the model can only be reused with the Weka tool support. We have converted it into standard formats. 

Xplacer leverages Weka \cite{hall2009weka}, a Java-based machine learning toolkit with a collection of machine learning algorithms for data mining tasks, to generate the AI model. 
A decision tree representing the AI model for Xplacer can be exported from Weka tool support.
Although the storage format for the model generated by Weka is proprietary \texttt{.model} format and the model can only be reused with the Weka tool support,
we can leverage HPC ontology to describe the Weka workflow and enhance the FAIRness for the Weka workflow.
Ideally, the offline learning with Weka can be replaced by an implementation using \texttt{scikit-learn (sklearn)}~\cite{sklearn}, a machine learning framework in Python, and later be converted into ONNX format~\cite{sklearn-onnx}.
The decision tree exported from the AI models generated by Weka can be annotated 
To improve the FAIRness for the AI Model used by Xplacer, we extend HPC Ontology support in order to annotate the decision tree following the annotation approach for Xpacer dataset.

\paragraph{Enhanced HPC Ontology for AI Models}
The original HPC Ontology does not have concepts and properties for internal details of a decision tree. As shown in Table~\ref{tab:hpcontology-decisiontree }, we have added a set of new concepts and properties to fill in the blank. 

\begin{table*}[!htp]\centering
\caption{Supplemental HPC Ontology to Annotate Decision Trees}\label{tab:hpcontology-decisiontree }
\scriptsize
\begin{tabular}{|l|l|l|}\toprule
\multicolumn{3}{|c|}{DecisionTree} \\ \hline
\textbf{Property } &\textbf{Data Type} &\textbf{Description} \\\midrule
name & xsd:string & name of the decision tree \\
wasDerivedFrom &xsd:string or xsd:anyURI & training datasets this call graph was derived from \\
decisionTreeNode &xsd:anyURL &link to one or more nodes of this decision tree \\ \hline
\multicolumn{3}{c}{DecisionTreeNode} \\ \hline
\textbf{Property } &\textbf{Data Type} &\textbf{Description} \\ \hline
treeNodeLevel &xsd:integer &level from 0 \\
decisionFeature &xsd:string &feature for the condition's left operand \\
relationOp &xsd:anyURI or xsd:string &operator for the decision condition, such as hpc:GreaterOrEqalOp \\
relationValue &xsd:float &value as the right operand of the decision condition \\
hasChildNode &xsd:boolean &if this node has children or not \\
trueNode &xsd:anyURI &link to the decision tree node when condition evaluates to be true \\
falseNode &xsd:anyURI &link to the decision tree node when condition evaluates to be false \\
decisionLabel &xsd:string &decision label for a leaf node in a decision tree \\
\bottomrule
\end{tabular}
\end{table*}

\paragraph{The Annotated Decision Tree Model}
A decision tree is formed by a group of tree nodes, example shown in Figure~\ref{fig:decision_tree}.  A tree node can be an internal node representing a decision relationship, or a leaf node representation a decision label.  Listing~\ref{decisionTree} shows a subset of the JSON-LD file for the decision tree used by the XPlacer. 
An annotated internal tree node is shown in Listing~\ref{internalTreeNode}.
Different from the internal nodes, a leaf node, shown in Listing~\ref{leafTreeNode}, has no associated child nodes and has a valid decision label property presented in the annotation.



\begin{lstlisting}[captionpos=t, caption=DecisionTree JSON-LD example, label={decisionTree}]
{
"@id": "http://example.org/decisiontree/DT000001",
"@type": [
    "HPC-Ontology#DecisionTree"
],
"HPC-Ontology#decisionTreeNode": [
    {
        "@id": "XPlacer1"
    },
    {
        "@id": "XPlacer2"
    },
...
]
}
\end{lstlisting}

\begin{lstlisting}[captionpos=t, caption=Internal DecisionTreeNode JSON-LD example, label={internalTreeNode}]
{
"@id": "Xplacer1",
"@type": [
    "HPC-Ontology#DecisionTreeNode"
],
"https://github.com/HPC-FAIR/HPC-Ontology#DecisionTree": [
    {
        "@value": "Xplacer"
    }
],
"HPC-Ontology#decisionFeature": [
    {
        "@value": "Block Size "
    }
],
"HPC-Ontology#falseNode": [
    {
        "@id": "Xplacer3"
    }
],
"HPC-Ontology#hasChildNode": [
    {
        "@value": true
    }
],
"HPC-Ontology#relationOp": [
    {
        "@value": "<="
    }
],
"HPC-Ontology#relationValue": [
    {
        "@type": "http://www.w3.org/2001/XMLSchema#float",
        "@value": "0.354839"
    }
],
"HPC-Ontology#treeNodeLevel": [
    {
        "@value": 0
    }
],
"HPC-Ontology#trueNode": [
    {
        "@id": "Xplacer2"
    }
]
},
\end{lstlisting}

\begin{lstlisting}[captionpos=t, caption=leaf DecisionTreeNode JSON-LD example, label={leafTreeNode}]
{
"@id": "Xplacer245",
"@type": [
    "HPC-Ontology#DecisionTreeNode"
],
"HPC-Ontology#DecisionTree": [
    {
        "@value": "Xplacer"
    }
],
"HPC-Ontology#decisionLabel": [
    {
        "@value": "1"
    }
],
"HPC-Ontology#hasChildNode": [
    {
        "@value": false
    }
],
"HPC-Ontology#treeNodeLevel": [
    {
        "@value": 12
    }
]
}
\end{lstlisting}

\end{comment}

%\subsection{Final FAIRness Assessment}
\noindent\textbf{Final FAIRness Assessment:}
The final FAIRness evaluation by the hybrid evaluation reveals a 83.0\% score after the improvements. Figure~\ref{fig:finalEval} presents the final statistics (Figure~\ref{fig:finalEvalA}) and the visual report showing the maturity level for each indicator according to the RDA manual evaluation (Figure~\ref{fig:finalEvalB}). 

%(76.6\% 36 out of 47 full score).  
%The final FAIRness evaluation using F-UJI reveals a 79\% fulfillment after the improvements.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!ht]
     \centering
     \hspace{-0.1in}
    \begin{minipage}{.45\linewidth}
        \begin{subfigure}[t]{.9\linewidth}
            \includegraphics[scale=0.3]{./figures/fig3_1.png}
            %\caption{Detail van een route}
            %\label{fig:weather_filter1}
        \end{subfigure} 
        \begin{subfigure}[b]{.9\linewidth}
            \includegraphics[scale=0.3]{./figures/fig3_2.png}
           \caption{Final FAIRness score}
        \label{fig:finalEvalA}
        \end{subfigure} 
        
    \end{minipage}
     \hspace{-0.1in}
     \begin{minipage}{.52\linewidth}
            \begin{subfigure}[t]{.9\linewidth}
                \includegraphics[scale=0.3]{./figures/fig3_3.png}
                \caption{Final FAIRness maturity levels}
                \label{fig:finalEvalB}
            \end{subfigure}
        \end{minipage}
        \caption{Final hybrid assessment}
        \label{fig:finalEval}
        \vspace{-0.1in}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The results show that the dataset does not fulfill FsF-I1-02M that requires namespaces of known semantic resources to be  present in the metadata of an object.  This is due to the limited support by the data hosting service by Zenodo to provide  namespaces for specific semantic resources.
A partial fulfillment is reported by F-UJI for FsF-R1-01MD that requires metadata for technical properties of the data file. We find that this is due to the implementation limitations on both F-UJI and Zenodo after investigation.  
The metric is considered fulfilled in our final manual assessment.
Another partial fulfillment report is for FsF-R1.2-01M that requires provenance metadata provided in a machine-readable version of PROV-O or PAV. 
We encoded the provenance information for XPlacer dataset at the fine-level granularity through HPC ontology and link to PROV-O ontology.  
However, these provenance metadata cannot be annotated into Zenodo's registry due to its limited support. This metric is also considered passed in our manual assessment.
%With the manual inspection and assessment, we can adjust the fulfillment score to 39 out of 47, that is 83\% of FAIRness fulfillment based on the hybrid evaluation. 

%The manual assessment is also conducted in the final assessment to evaluate the FAIRness fulfillment for the fine-grain data (Fig.~\ref{fig:RDAFinalEval}). 
The final assessment shows that the use of the HPC ontology significantly improves the metadata support for the XPlacer dataset, resulting in full fulfillment for all FAIRness indicators for `F and A' FAIR principles.  
%With current support from the HPC ontology, the data and metadata do not include qualified references to other data or metadata.  
However, providing full and qualified references to other data standards is still ongoing development for the HPC ontology.  This leads to a lower fulfillment, in implementation phase, for RDA-I3-01D (Data includes references to other data), RDA-I3-02D (Data includes qualified references to other data), and RDA-I3-04M (Metadata include qualified references to other data).
In the `R' FAIR principle, RDA-R1.2-02M (Metadata includes provenance information according to a cross-community languages) is also considered in implementation phase to support PROV-O ontology as the cross-community languages for provenance information.  
There is no community standard specified for data and metadata in HPC community.  We propose to use the HPC ontology as one metadata standard for HPC.
As HPC ontology is still under development, we consider RDA-R1.3-01M, RDA-R1.3-01D, RDA-R1.3-02M and RDA-R1.3-02D still in the implementation phase. %\todo{HPC ONTOLOGY has been released as a draft standard. We should give some credits to it. Would a middle level score like 3/5 be fair???}


%


\begin{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.35\textwidth}
         \centering
\includegraphics[scale=0.35]{./figures/Final_Eval.png}
        \caption{Final FAIRness score}
                \label{fig:finalEvalA}
\end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.55\textwidth}
         \centering
 \includegraphics[scale=0.35]{./figures/RDA-Eval-final.pdf}
     \caption{Final assessment FAIRness maturity levels}
             \label{fig:finalEvalB}
     \end{subfigure}
     \hfill
        \caption{Final hybrid assessment}
        \label{fig:finalEval}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{comment}




\begin{comment}
\begin{figure}[!htbp]
%\vspace{-0.15in}
 \centering
 %\vspace{-0.05in}
 \includegraphics[scale=0.25]{./figures/FUJI-final.pdf}
 %\vspace{-0.2in}
 \caption{\textmd{Result after metadata update. \todo{you may want to show the adjusted 95.8\% number instead, somehow.}}}
 \label{fig:FUJIFinalEval}
%\vspace{-0.15in} 
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!htbp]
%\vspace{-0.15in}
 \centering
 %\vspace{-0.05in}
 \includegraphics[scale=0.35]{./figures/RDA_final.pdf}
 %\vspace{-0.2in}
 \caption{\textmd{RDA result after metadata update.}}
 \label{fig:RDAFinalEval}
%\vspace{-0.15in} 
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\todo{reference https://about.zenodo.org/principles/ to justify the final scores}

\end{comment}


\begin{comment}
\begin{enumerate}[leftmargin=*] 
    \item []Findability: The enhancements add a permanent DOI provided by Zenodo.  The new dataset, converted from CSV into JSON-LD format, has the persistent metadata describing the data provided from HPC ontology.  All the metadata from HPC ontology is considered comprehensive data to have  a globally unique URIs, descriptions, provenance information describing the creator/submitter of the data, machine-actionable license information and links to associated information.  The dataset is stored at one place and can be discoverable through multiple registries.  The highest fulfillment for findability can be achieved with the the enhancements applied to Xplacer dataset and AI models.
    \item []Accessability:
    The HPC ontology, once publicly released and with DOI obtained, will provide permanent metadata information for the Xplacer dataset and AI models. This enhancement drives to the full fulfillment for datta accessability.
    \item []Interoperatbility:
    JSON-LD format, the new format converted from the CSV raw data, for Xplacer dataset is a structured format that can be machine-actionable through query language support.  Adopting JSON-LD for datasett fulfills the first assessment for data interoperability.
    The HPC ontology defines vocabularies and schema specifically needed in HPC field.  Schema used for general purposes or other domains can be obtained by the linkage among HPC ontology and other public ontologies.
    Therefore, the vocabularies and schema used to describe the Xplacer dataset and AI models are open and universal discoverable with global identifiers linking to their explanations. All the metadata information can be linked with unique URIs through HPC ontology. 
    The data interoperability defined for FAIR principles can be fulfilled with the enhancements applied.
    \item []Reusability:
    Fulfilling reusability principle requires  a clear machine-readable licence and provenance information on how the data was formed. 
    We achieve the fulfillment by applying creative common license for the dataset, AI models, and ontologies to define the usage rights for Xplacer dataset. 
    Meanwhile, HPC ontology sub classes and properties jointly encode  provenance information to describe the source information of the data and details describing the methodologies and workflows by which the data is produced.
    
\end{enumerate}
\end{comment}





==> TEML'22 FAIRness-Extended-arXiv/introduction.tex <==
%Artificial intelligence (AI) is being rapidly applied to various research domains in recent years. 
Research activities in high-performance computing (HPC) community have applied machine learning (ML) for various research needs such as performance modeling and prediction~\cite{lopez2014survey}, %singh2007predicting, sun2017automated,malakar2018benchmarking
memory optimization~\cite{xu2019machine, xunified}, and so on. %
A typical ML-enabled HPC study generates a large amount of valuable datasets from the HPC experiment outputs. The datasets serve as training inputs for the ML models applied in research. 
There is an increasing awareness of the need for data reuse in HPC community.
%The magnitude of data that can be produced in HPC community should greatly benefit the ML research need for large scale dataset.
However, the community still lacks guidelines and experiences to effectively access and share the data that was collected in various research experiments.


The FAIR Guiding Principles~\cite{wilkinson2016fair} were published to advocate the reuse of data and other digital contents, including algorithms, software tools, source codes, and workflows that led to the generation of data.
These principles serve as a guideline, but not specification, to make digital data and contents findable, accessible, interoperable, and reusable by both humans and machines.
The FAIR principles have been broadly adopted in certain research communities, such as biomedical and health science, with a range of studies and implementations to address the challenges in achieving data FAIRness.
Many recommendations and best practices are documented to prepare FAIR data in specific research domains.
There are also various initiatives and active community activities, focusing the generalist, started to promote the importance of data FAIRness and assist to FAIRify the existing datasets. 
However, these principles and practices haven’t yet been tailored to benefit the HPC community. 

In this paper, we present a methodology and a case study to make HPC machine learning training datasets FAIR, in the domain of machine learning-based program analyses and optimizations for HPC.
We investigate the needs and challenges to FAIRify a HPC dataset following the established data FAIRification workflows used in other research communities.
Seeing limitations of existing FAIRness evaluation approaches, we propose a hybrid assessment step with both manual and automated assessments. Concrete actions are then suggested to address missing features in the chosen dataset. The methodology is evaluated using a representative dataset, demonstrating significant FAIRness improvement from 19.1\% to 83.0\%. 

This paper has the following contributions:
\begin{itemize}
    \item We survey the best practices and approaches to make datasets FAIR, including those for FAIRness assessment and improvements (or FAIRification). 
    \item A comprehensive, quantitative methodology is proposed to evaluate and improve FAIRness of HPC datasets. 
    \item The methodology leverages a hybrid assessment to generate a single FAIRness score. An ontology is developed to help address common issues for FAIRness improvement. 
    \item Using a concrete dataset, we evaluate the proposed methodology for its effectiveness.
%    \item We also highlight common issues and solutions to make HPC data FAIR. 
%    \item We formulate a detailed process customized for HPC datasets and AI models. \todo{needs to confirm if we actually could do this}
\end{itemize}

The remainder of this paper is organized as follows: Section \ref{FAIR} gives background information about the FAIR principles. % recommended FAIRification processes and the data FAIRness evaluation.
Section \ref{Fairify} discusses the methodology we design to evaluate and improve FAIRness of HPC datasets and ML models.
Section \ref{dataset} presents an example dataset and an example ML model generated from a prior project named XPlacer \cite{xu2019machine}. Experiment results are shown in Section~\ref{results}.  Section \ref{relatedwork} summarizes the related work and section \ref{conclusion} concludes this paper.

==> TEML'22 FAIRness-Extended-arXiv/methodology.tex <==
%\todo{We should give a name to the methodology.}

We propose a new methodology to improve the FAIRness of HPC datasets. The method has three steps: 1) initial FAIRness assessment, 2) improving FAIRness based on assessment results, and 3) final assessment. We elaborate the first two steps since the last step is a repetition of the first one.  

\subsection{Initial FAIRness Assessment}
After surveying the existing FAIRness evaluation methods, we have found that while
the questionnaire-based manual evaluations have advantages to cover more details, the manual input process and the tendency to cause biased result are not ideal (shown in Table~\ref{tab:manualVsAuto}).
On the other hand, automated evaluation avoids manual intervention and biased result.  But they are less flexible and limited by the implementation for supported data granularity and metadata. 
As a result, we propose a hybrid approach involving both manual and automated assessments to have a more productive, flexible and informative evaluation.
%Table~\ref{tab:manualVsAuto} shows the high-level differences between these two approaches.
%We also observed the automated evaluation is preferred and is superior in its ease of use. But automated evaluation lacks the complete coverage for full details in the FAIR Guiding Principles.
%The advantages of the manual evaluation, for good coverage for FAIR Guiding Principles, can compensate the drawbacks in the automated approach.  
%Manual evaluation also provides flexibility to evaluate FAIRness of data of different granularity, ranging from metadata, datasets, to data elements.
%To achieve a better FAIRness evaluation, we propose a hybrid evaluation approach to leverage the strengths from both the manual and automated evaluation approaches.
%\todo{swap the order of manual vs. automate evaluations in the text to match the order we actually use them.}

We choose the FAIRness assessment service by F-UJI \cite{DEVARAJU2021100370} as the automated evaluation service due to many desirable features it has.
%We expect that the automated evaluation will gradually improve the coverage for better and easier FAIRness evaluation process.
The F-UJI service designs 17 FAIRness metrics, derived from the 41 RDA FAIRness maturity indicators, that can be evaluated with automatic testings. 
It uses a scoring system to provide quantitative evaluation result, in percentage,  reflecting the ratio of the achieved score number to the full score number. 
%F-UJI has two highlights compared to other automated FAIRness evaluation services.  
Moreover,  F-UJI provides detailed output to each metric evaluation as a guidance to assist users to improve the FAIRness maturity. Finally, F-UJI is an open-source project that can be expanded to include new features and support to address specific needs for HPC community.
However,  F-UJI has insufficient support for many FAIR Guiding Principals related to metadata. 
%Therefore it is suitable to obtain an overview of the FAIRness maturity. 

\begin{table*}[!htbp]
	\centering
\begin{tabular}{|l|l|l|l|} \hline
\textbf{Criteria} & \textbf{Description} &\textbf{Manual}  & \textbf{Automated} \\ \hline
Metadata  & Metadata information that can be evaluated & Flexible  & Fixed \\  \hline
Productivity & Human effort required for evaluation & Low  &  High \\ \hline
Completeness & FAIR Guiding Principles coverage & High & Low 	\\ \hline
%Multi-
Granularity & Data granularity that can be evaluated & Yes &  No \\ \hline
\end{tabular}
\caption{Comparison of manual and automated assessment.
}
\label{tab:manualVsAuto}
\end{table*}

\begin{comment}

%we conducted an initial FAIRness assessment for Xplacer dataset using an automated evaluation provided by F-UJI \cite{F-UJI}. 
\begin{itemize}[leftmargin=*]
    \item The evaluation metrics are derived from the same list of FAIRness indicators used in the manual evaluation service from RDA.
    %\item The automated evaluation is superior to the questionnaire-based evaluation by eliminating manual information submission step and reducing the evaluation bias impacted by the provided evaluation information.
    %\item F-UJI collects seventeen metrics to cover the evaluations for most FAIR principles and sub-principles. Metrics to evaluate principles A2 and I2 are not available in F-UJI.
    \item F-UJI uses a scoring system to provide quantitative evaluation result, in percentage reflecting the ratio of the achieved score number to the full score number.
    \item F-UJI provides detailed output and debug messages to each metric evaluation as guidance to assist users to improve the FAIRness maturity.  
    \item The F-UJI implementation is an open-source project that can be expanded to include new features and support to address specific needs for HPC community.
\end{itemize}
 However, F-UJI does not sufficiently support some principals, especially for metadata. Therefore it is suitable to obtain an overview of the FAIRness maturity. 

\end{comment}

%\todo{cite and name the manual approach,  and clarify if it is discrete vs. open-answer questionnaire based}. 
The self-assessment tool by RDA FAIR data maturity model is chosen as the manual evaluation approach. It uses the same 41 RDA FAIRness maturity indicators referenced by F-UJI.
%Both also share the same definitions for FAIRness maturity. 
%FAIRness evaluation  with three levels of priority specified (essential, important and useful) to cover all FAIR Guiding Principles. 
This manual assessment is a discrete-answer questionnaire-based evaluation. Users provide an answer, with an associated level number, to each indicator from one of the following options to determine the maturity: (0) not applicable; (1) not been considered; (2) under consideration or in planning; (3) in implementation; and (4) fully implemented.  Visualized report is available from the tool to present the maturity of the FAIRness. The manual evaluation provides good coverage for the details in the FAIR principles and can present the full details of the FAIRness readiness. 
It also provides flexibility to evaluate FAIRness of data of different granularity, ranging from metadata, datasets, to data elements. However, manually checking each indicator to evaluate given data is tedious and error-prone. 

The RDA indicators and F-UJI metrics share the same notation with three components to name their IDs:
(1) the project abbreviation, RDA or FsF (FAIRsFAIR: the parent project of F-UJI); (2) the related FAIR Guiding Principle identifier (e.\,g. F1); and (3) a local identifier number with a suffix encoding to identify resource that will be evaluated: metadata (M), data (D), or both (MD).  

In the proposed hybrid assessment, we consolidate 41 RDA indicators and 17 F-UJI metrics to form a new list of 47 indicators as shown in Table~\ref{tab:fairness}.
There are 11 indicators
, marked $\ast$ in Table~\ref{tab:fairness}, 
originated from both RDA indicators and F-UJI metrics, e.\,g. RDA-F1-01D and FsF-F1-02D. % because the F-UJI metric is derived from the RDA maturity indicators without any revision in the descriptions.  
%For example, the RDA-F1-01D and FsF-F1-02D both evaluate if data is identifiable by a persistent identifier.  
The hybrid evaluation for these 11 indicators will take the result from the F-UJI metric because the automated test has the advantage to avoid biased result. 

%It can be easily seen in Table~\ref{tab:fairness} that original RDA indicators provide full coverage for FAIR Guiding Principles.
%F-UJI metrics bring in advantages of testing to avoid biased results.
To generate quantitative assessment results, we design a scoring system as follows: each indicator is given one point if its result is determined by the RDA maturity indicator as fully implemented, or by the F-UJI metric as a fully passed test. A total of 47 points for the whole hybrid evaluation consist 8 points for 'F', 13 points for 'A', 14 points for 'I' and 12 points for 'R', where the points correspond to the number of FAIRness indicators for each FAIR principle.
%\MK{Is this split of points determined by F-UJI?} 
The final score is represented as the percentage of the earned points divided by the total point count. 
%\todo{I added this final score is a percentage.. please check correctness}


%In our initial and final assessment steps, we leverage the advantage of the automated evaluation by first conducting the evaluation using F-UJI to obtain the summary report. Afterward, we manually perform the manual evaluation to inspect the details not covered by the automated approach to complete the FAIRness assessment.

%\todo{It is not clear how to combine auto + manual evaluation methods to derive a final score for our own hybrid method. This may be a key contribution. Or we just watch two numbers separately?}

%\todo{move the text about relative metrics to this section. }


\begin{table*}[!htp]\centering
\caption{FAIR Guiding Principles: maturity indicators and assessment metrics}
\label{tab:fairness}
\scriptsize
\begin{threeparttable}[b]
\begin{tabular}{|l|l|p{10cm}|c|} \hline
\textbf{P\tnote{1}}& \textbf{Indicator} &\textbf{Description} & \textbf{S\tnote{2}} \\ \hline

\multirow{6}{*}{\hfil F1} & RDA-F1-01M & Metadata is identified by a persistent identifier & \multirow{6}{*}{\hfil 4}\\
\cline{2-3}

& RDA-F1-01D \tnote{*} & \multirow{2}{*}{Data is identified by a persistent identifier} & \\

& FsF-F1-02D & & \\
\cline{2-3}

& RDA-F1-02M & Metadata is identified by a globally unique identifier & \\
\cline{2-3}

& RDA-F1-02D \tnote{*}& \multirow{2}{*} {Data is identified by a globally unique identifier} & \\

& FsF-F1-01D & &\\
\hline
\multirow{2}{*}{\hfil F2} & RDA-F2-01M &  Rich metadata is provided to allow discovery & \multirow{2}{*}{\hfil 2} \\
\cline{2-3}

& FsF-F2-01M & Metadata includes descriptive core elements to support data findability &\\
\hline

\multirow{2}{*}{\hfil F3} & RDA-F3-01M \tnote{*}&  \multirow{2}{*}{Metadata includes the identifier for the data} & \multirow{2}{*}{\hfil 1} \\
& FsF-F3-01M & & \\
\hline

\multirow{2}{*}{\hfil F4}  & RDA-F4-01M \tnote{*}&  \multirow{2}{*}{Metadata is offered in such a way that it can be harvested and indexed} & \multirow{2}{*}{\hfil 1} \\

&FsF-F4-01M & &\\
\hline
\hline

\multirow{11}{*}{\hfil A1} & RDA-A1-01M &  Metadata contains information to enable the user to get access to the data & \multirow{11}{*}{\hfil 9}\\

\cline{2-3}

 & RDA-A1-02M &  Metadata can be accessed manually &\\
 
\cline{2-3}

& RDA-A1-02D &  Data can be accessed manually & \\
 
\cline{2-3}

 & RDA-A1-03M &  Metadata identifier resolves to a metadata record or digital object & \\

\cline{2-3}

& RDA-A1-03D &  Data identifier resolves to a metadata record or digital object  &\\

\cline{2-3}
 & RDA-A1-04M \tnote{*}& \multirow{2}{*}{Metadata is accessed through standardised protocol}& \\
&FsF-A1-02M && \\

\cline{2-3}
 & RDA-A1-04D \tnote{*}&  \multirow{2}{*}{Data is accessed through standardized protocol} &\\
& FsF-A1-03D &  &\\
\cline{2-3}

& RDA-A1-05D &  Data can be accessed automatically &\\

\cline{2-3}
& FsF-A1-01M & Metadata contains access level and access conditions of the data &\\

\hline
\multirow{2}{*}{\hfil A1.1} & RDA-A1.1-01M &  Metadata is accessible through a free access protocol &\multirow{2}{*}{\hfil 2} \\

\cline{2-3}

 & RDA-A1.1-01D &  Data is accessible through a free access protocol & \\

\hline

A1.2 & RDA-A1.2-01D &  Data is accessible through an access protocol that supports authentication and authorization & \multirow{2}{*}{\hfil 1} \\
\hline

\multirow{2}{*}{\hfil A2}  & RDA-A2-01M \tnote{*} &  \multirow{2}{*}{Metadata is guaranteed to remain available after data is no longer available} & \multirow{2}{*}{\hfil 1}\\

&FsF-A2-01M& &\\
\hline
\hline

\multirow{6}{*}{\hfil I1} & RDA-I1-01M &  Metadata uses knowledge representation expressed in standardized format & \multirow{6}{*}{\hfil 6}\\

\cline{2-3}

& RDA-I1-01D &  (Data uses knowledge representation expressed in standardized format &\\

\cline{2-3}
 & RDA-I1-02M &  Metadata uses machine-understandable knowledge representation  &\\
 
\cline{2-3}
 & RDA-I1-02D &  Data uses machine-understandable knowledge representation  &\\
 
 \cline{2-3}
 &FsF-I1-01M & Metadata is represented using a formal knowledge representation language &\\
 \cline{2-3}
 &FsF-I1-02M & Metadata uses semantic resources &\\
 \hline
 
 \multirow{2}{*}{\hfil I2}  & RDA-I2-01M &  Metadata uses FAIR-compliant vocabularies   & \multirow{2}{*}{\hfil 2}\\

 \cline{2-3}

 & RDA-I2-01D &  Data uses FAIR-compliant vocabularies & \\
 \hline

\multirow{7}{*}{\hfil I3} & RDA-I3-01M \tnote{*}&  \multirow{2}{*}{Metadata includes references to other (meta)data} & \multirow{7}{*}{\hfil 6}\\

&FsF-I3-01M& & \\
\cline{2-3}

& RDA-I3-01D &  Data includes references to other (meta)data & \\
\cline{2-3}
& RDA-I3-02M &  Metadata includes references to other data & \\

\cline{2-3}
& RDA-I3-02D &  Data includes references to other data &  \\

\cline{2-3}

& RDA-I3-03M &  Metadata includes qualified references to other metadata  & \\

\cline{2-3}

& RDA-I3-04M &  Metadata include qualified references to other data & \\

\hline
\hline

\multirow{3}{*}{\hfil R1} & RDA-R1-01M &  Plurality of accurate and relevant attributes are provided to allow reuse & \multirow{2}{*}{\hfil 2} \\
\cline{2-3}

&FsF-R1-01MD & Metadata specifies the content of the data & \\
\hline

\multirow{4}{*}{\hfil R1.1} & RDA-R1.1-01M & Metadata includes information about the license under which the data can be reused & \multirow{4}{*}{\hfil 3}\\

\cline{2-3}
& RDA-R1.1-02M &  Metadata refers to a standard reuse license & \\
\cline{2-3}
 & RDA-R1.1-03M \tnote{*}&  \multirow{2}{*}{Metadata refers to a machine-understandable reuse license} & \\
& FsF-R1.1-01M & & \\% Metadata includes license information under which data can be reused.\\
\hline
\multirow{3}{*}{\hfil R1.2} & RDA-R1.2-01M &  Metadata includes provenance information according to community-specific standards & \multirow{3}{*}{\hfil 3} \\

\cline{2-3}

& RDA-R1.2-02M &  Metadata includes provenance information according to a cross-community language & \\

\cline{2-3}

&FsF-R1.2-01M & Metadata includes provenance information about data creation or generation & \\
\hline

\multirow{6}{*}{\hfil R1.3} & RDA-R1.3-01M \tnote{*}&  \multirow{2}{*}{Metadata complies with a community standard } & \multirow{6}{*}{\hfil 4}\\
&FsF-R1.3-01M & &\\
\cline{2-3}
& RDA-R1.3-01D &  Data complies with a community standard & \\

\cline{2-3}

& RDA-R1.3-02M &  Metadata is expressed in compliance with a machine-understandable community standard & \\
\cline{2-3}

& RDA-R1.3-02D \tnote{*}&  \multirow{2}{*}{Data is in compliance with a machine-understandable community standard} &\\
&FsF-R1.3-02D & &\\

\hline


\end{tabular}
\begin{tablenotes}
    \item[1] FAIR Guiding Principle ID
    \item[2] Max score allocated to each sub-principle
    \item[*] Both RDA FAIRness indicator and F-UJI metric represent the same evaluation
  \end{tablenotes}
 \end{threeparttable}

\end{table*}


\begin{comment}
\begin{table*}[!htp]\centering
\caption{FAIR Principles (PRIN.): maturity indicators and assessment metrics}
\label{tab:fairness}
\scriptsize
\begin{tabular}{|p{.75cm}|l|p{5.5cm}||l|p{5.5cm}|} \hline
\textbf{PRIN.}& \textbf{RDA Indicator} &\textbf{Indicator Description}  & \textbf{F-UJI Metric} &\textbf{Metric Description} \\ \hline

\multirow{2}{*}{\hfil F1} & RDA-F1-01M/D & (Meta)data is identified by a persistent identifier & FsF-F1-01D & Data is assigned a globally unique identifier \\
\cline{2-5}

 & RDA-F1-02M/D & (Meta)data is identified by a globally unique identifier  & FsF-F1-02D & Data is assigned a persistent identifier\\
\hline

F2 & RDA-F2-01M &  Rich metadata is provided to allow discovery & FsF-F2-01M & Metadata includes descriptive core elements to support data findability\\
\hline

F3 & RDA-F3-01M &  Metadata includes the identifier for the data & FsF-F3-01M & Metadata includes the identifier of the data it describes \\
\hline

F4 & RDA-F4-01M &  Metadata is offered in such a way that it can be harvested and indexed &  FsF-F4-01M & Metadata is offered in such a way that it can be retrieved by machines\\
\hline

\multirow{5}{*}{\hfil A1} & RDA-A1-01M &  Metadata contains information to enable the user to get access to the data &  \multirow{5}{*}{\makecell{FsF-A1-01M \\ FsF-A1-02M \\ FsF-A1-03D }} & \multirow{5}{*}{\makecell{Metadata contains access level and access conditions of the data \\ Metadata is accessible through a standardized communication protocol \\ Data is accessible through a standardized communication protocol }}
\\
\cline{2-3}

 & RDA-A1-02M/D &  (Meta)data can be accessed manually  &  &  \\
\cline{2-3}

 & RDA-A1-03M/D &  (Meta)data identifier resolves to a metadata record or digital object & &   \\
\cline{2-3}

 
 & RDA-A1-04M/D &  (Meta)data is accessed through standardised protocol &  & \\
\cline{2-3}

 & RDA-A1-05D &  Data can be accessed automatically &  & \\
\hline

A1.1 & RDA-A1.1-01M/D &  (Meta)data is accessible through a free access protocol  & N/A  &\\
\hline

A1.2 & RDA-A1.2-01D &  Data is accessible through an access protocol that supports authentication and authorisation  & N/A & \\
\hline

A2 & RDA-A2-01M &  Metadata is guaranteed to remain available after data is no longer available  & FsF-A2-01M & Metadata remains available, even if the data is no longer available.\\
\hline

\multirow{2}{*}{\hfil I1} & RDA-I1-01M/D &  (Meta)data uses knowledge representation expressed in standardised format  & FsF-I1-01M & Metadata is represented using a formal knowledge representation language \\
\cline{2-5}

 & RDA-I1-02M/D &  (Meta)data uses machine-understandable knowledge representation  & FsF-I1-02M & Metadata uses semantic resources \\
\hline

I2 & RDA-I2-01M/D &  (Meta)data uses FAIR-compliant vocabularies  & N/A & \\
\hline

\multirow{4}{*}{\hfil I3} & RDA-I3-01M/D &  (Meta)data includes references to other (meta)data & \multirow{4}{*}{FsF-I3-01M} & \multirow{4}{*}{Metadata includes links between the data and its related entities} \\
\cline{2-3}

 & RDA-I3-02M/D &  (Meta)data includes references to other data &  & \\
\cline{2-3}

 & RDA-I3-03M &  Metadata includes qualified references to other metadata &  & \\
\cline{2-3}

 & RDA-I3-04M &  Metadata include qualified references to other data &  & \\
\hline

R1 & RDA-R1-01M &  Plurality of accurate and relevant attributes are provided to allow reuse   & FsF-R1-01MD & Metadata specifies the content of the data.\\
\hline

\multirow{3}{*}{\hfil R1.1} & RDA-R1.1-01M & Metadata includes information about the license under which the data can be reused  & \multirow{3}{*}{FsF-R1.1-01M} & \multirow{3}{*}{Metadata includes license information under which data can be reused.}  \\
\cline{2-3}

 & RDA-R1.1-02M &  Metadata refers to a standard reuse license &  & \\
\cline{2-3}

 & RDA-R1.1-03M &  Metadata refers to a machine-understandable reuse license &  & \\
\hline

\multirow{2}{*}{\hfil R1.2} & RDA-R1.2-01M &  Metadata includes provenance information according to community-specific standards & \multirow{2}{*}{FsF-R1.2-01M} & \multirow{2}{*}{Metadata includes provenance information about data creation or generation.}\\
\cline{2-3}

 & RDA-R1.2-02M &  Metadata includes provenance information according to a cross-community language &  & \\
\hline

\multirow{2}{*}{\hfil R1.3} & RDA-R1.3-01M/D &  (Meta)data complies with a community standard & \multirow{2}{*}{FsF-R1.3-02D} & \multirow{2}{*}{Metadata follows a standard recommended by the target research community of the data} \\
\cline{2-3}

 & RDA-R1.3-02M/D &  (Meta)data is expressed in compliance with a machine-understandable community standard &  &\\
\hline

\end{tabular}
\end{table*}

\end{comment}


\subsection{Improving FAIRness}
\label{sec:improvingMethods}
%The assessment score, consisting results from both manual and automated evaluation, presents a quantitative indication for the FAIRness of selected data.
Improving the FAIRness can be achieved by systematically addressing issues reported by the manual and automated assessments.
%Given no strict tests used in the manual assessment, users evaluate the FAIRness according to their own justifications.  Based on the same justifications, users can enhance the FAIRness by addressing the missing features.
%The F-UJI evaluation service provides four maturity levels, incomplete, initial, moderate, and advanced, to summarize the assessment result for each F-UJI metric.
%For example, the F-UJI evaluation provides detailed reports of the tests, test results and debug information applied to the metrics.  
  %Users can obtain a DOI to address this warning. %  After the enhancement, F-UJI will then report the maturity level for metric FsF-F1-02D as advanced and show the debug message: "SUCCESS: Persistence identifier scheme -: doi".
%There is no fixed list of tasks to improve FAIRness for all datasets.  The remedy to enhance FAIRness varies with the features and contents in the dataset.
Users can iterate through all the metrics that are not marked as fully implemented or passed. The evaluation reports often give reasons for the failed tests associated with the metrics. 
Due to page limit, we present example actions users can take to address some commonly seen inadequacies in FAIRness revealed by our hybrid assessment process. 
We also label these actions by identifiers with a prefix MT (abbreviation for method). 

\begin{itemize}[leftmargin=*]
\item \textit{Getting persistent identifier} (MT-PID):
%A dataset using URL as its global identifier will trigger F-UJI to mark the metric FsF-F1-02D as incomplete with a message: "WARNING: Not a persistent identifier scheme -: url". 
It is straightforward for a data collector to use the web address (URL) as the identifier for a dataset.  However, URLs tend to change over time which leads to broken links to the data. 
A persistent and unique identifier, such as digital object identifier (DOI), is the preferred identifier for a FAIR dataset.
%There are numerous data hosting services (such as w3id.org) providing DOIs service for general or domain-specific usages.
It is recommended to register the dataset at general or domain-specific registry systems to make the data more discoverable.
%There are several ways to get a DOI as a persistent identifier a dataset. For dataset hosted at the public repository like Github.com , a DOI can be obtained by pushing the registering a release version to  Zenodo\cite{zenodo}.  
We select Zenodo\footnote{https://zenodo.org/}, a general-purpose open access repository, as our default platform to generate DOIs. 
%It assigns DOIs to all publicly available uploads to make the uploaded contents citable.  It also supports data content harvesting via the OAI-PMH protocol.
%For other dataset hosted online with URLs, getting a permanent identifiers for the web locations, such as a registry from w3id.org, to replace URLs is the ideal option to have a persistent data identifier.  
%The persistent web identifier can be obtained from services like w3id.org.For the other types of datasets, 
%Datasets uploaded to Zenodo will have the general-purpose registry service provided. 
%The rest can seek for registry service provided in different scientific community.


\item \textit{Providing coarse-grain metadata information} (MT-coarse-metadata):
Inadequate metadata is a common issue for datasets to fulfill the FAIR principles.
Again, we use public data hosting services such as \texttt{zenodo.org} to leverage their  built-in metadata.  The metadata information are provided by filling in the required information during the data registering/uploading process.
This type of metadata tends to describe general information of the associated dataset.
Data collectors can also prepare metadata by following guidance for general data, e.\,g. Dublin Core metadata initiative, or domain-specific data, e.\,g. Data Documentation Initiative (DDI) for social, behavioral, economic and health sciences.
%(one example should be sufficient) a and Ecological Metadata Language (EML) for ecology community.
With manual FAIRness evaluation, users have greater flexibility to prepare the metadata.  Specific metadata formats and requirements should be fulfilled if the dataset is assessed by an automated evaluation service.
The F-UJI automated evaluation supports several multidisciplinary meatadata standards, e.\,g. Dublin Core and DataCite Metadata Schema, and metadata standards from several scientific domains, e.\,g. biology, botany, and paleontology.  General metadata information supported by \texttt{zenodo.org} are recognized by the F-UJI evaluation. 
%\todo{Question: Is zenodo.org metadata directly recognized by F-UJI? Please clarify this.}

\item \textit{Generating rich attributes for different granularity of data} (MT-fine-metadata). It is relatively easy to make a whole dataset FAIR. However, significant work is needed to make fine-grain data elements inside a dataset FAIR. There is a lack of community standards to provide rich attributes for the data elements of various science domains. In HPC, datasets can be generated from performance profiling tools, compilers, runtime systems with very different attributes. 
%AI models also have domain-specific internal properties. 
To address this problem, we are developing the HPC Ontology~\cite{liao2021hpc} to provide standard attributes which can be used to annotate fine-grain data elements in different subdomains of HPC, including GPU profiling results, program analysis (e.\,g. call graph analysis), and machine learning models (e.\,g. decision trees). The design of HPC Ontology is modular so it can be extended to include more subdomains in the future. %Table~\ref{tab:xplacer-properties} list examples of properties defined in HPC ontology and needed by the Xplacer dataset.  

\item \textit{Automatic annotating data elements} (MT-auto-annotating). Even with existing standard attributes, it is impractical to manually annotate data elements one by one. 
Since most datasets are published in CSV files, we leverage Tarql\footnote{https://tarql.github.io/}, a command-line tool for converting data stored in CSV files into the Resource Description Framework (RDF) format using standard metadata and attributes provided by the HPC Ontology. % by querying delimited files using SPARQL 1.1 syntax, to accomplish the format conversion.  

\item \textit{Provenance information} (MT-provenance):
Provenance information is required to fulfill `R' FAIR principle.
Similar to the metadata, basic provenance information such as publication date and publisher, can be provided through the data hosting service such as zenodo.org.  
Formal provenance metadata, such as PROV, is recommended for advanced provenance information support.


\item \textit{License information} (MT-license):
  Data collectors should choose and apply license information to the collected dataset to fulfill `R1.1' FAIR principle. A recommended choice for data is one of the Creative Commons license. 
  %It worth noting the license will define different rights to distribute the copyrighted work.  %Data collectors should pick the most appropriate license to fulfill the purposes of the collected data.

\end{itemize}

\begin{comment}


 A FAIR metadata has to have three important traits: 
 1) it has to be comprehensible and machine-actionable; 
 2) metadata needs to be persistent regardless of the existence of the data; 
 and 
 3) metadata needs to be linked to other data or metadata.  
 \todo{Link HPC ontology to other metadata}
 We investigate leveraging the rich information provided by ontologies to provide a complete support for FAIR metadata.
 To achieve the full fulfillment for FAIR metadata, a HPC ontology is proposed to collect the essential concepts and properties capturing information from the HPC domain. 
 HPC-specific vocabularies used to describe data and metadata can be retrieved within HPC ontology.
 Vocabularies for general purposes and other specific domains can be obtained from other public ontologies though the linkages from HPC ontology.  
 \end{comment}
 
%This is due to the reason that a URL is subject to change and not considered as a persistent identifier.  We can fix this simply by providing a persistent identifier, e.g. DOI \todo{Exactly how to generate DOI? Please mention a URL to do this. This is the purpose of this paper: provide concrete HOW-TOs for FAIRness so people don't need to search around}, representing the same Github repository.  The F-UJI will then report the maturity level for metric FsF-F1-02D as advanced and show the debug message: "SUCCESS: Persistence identifier scheme -: doi".

\begin{table*}[!htp]\centering
\caption{Examples of HPC Ontology properties to annotate fine-grain GPU profiling data elements}
\label{tab:xplacer-properties}
\scriptsize
\begin{tabular}{|l|l|l|}\hline
\textbf{Property} &\textbf{Data type} &\textbf{Description} \\\hline
hpc:benchmark & xsd:anyURI & Link to the associated benchmark software ID in ontology\\
hpc:kenelName & xsd:string & Kernel name\\
hpc:gpuThreadBlockSize & xsd:integer & Launch block size \\
hpc:registersPerThread & xsd:integer & Register usage per thread \\
hpc:gpuThreadCount & xsd:integer & Threads count in launched kernel \\
hpc:gpuWavesPerSM & xsd:integer & Wave count in SM \\
hpc:maxGPUThreadBlockSizeLimitedByRegister & xsd:integer & Max block limited by registers \\
hpc:maxGPUThreadBlockSizeLimitedByWarps & xsd:integer & Max block limited by warps \\
hpc:cpuPageFault & xsd:integer &  CPU page fault count\\
hpc:gpuPageFault & xsd:integer &  GPU page fault count\\
hpc:hostToDeviceTransferSize & qudt:QuantityValue & Host to Device data transfer size \\
hpc:deviceToHostTransferSize & qudt:QuantityValue & Device to Host data transfer size\\

\hline
\end{tabular}
\end{table*}


\todo{We should include some details about how we develop metadata (HPC Ontology), how to annotate existing datasets with metadata, etc.  Again , a table listing principles/metrics and how to improve the relevant metrics is best with concrete steps/URLs readers can follow.}

\begin{comment}
% we already say in the beginning that the last step is a repetition of the first one
% and only first two steps are elaborated in this section

\subsection {Final Assessment}
Once enhancements are made into the dataset to improve the maturity of FAIRness, users can use go through another assessment process to check if the enhancements are effective to improve the FAIRness.
It could take multiple iterations of revision to enhance the dataset to achieve the highest maturity from the F-UJI assessment. \todo{Again, why is only F-UJI assessment mentioned here?  We should refer to our hybrid assessment method.}



The proposed methodology to improve FAIRness for HPC dataset and  AI  models leverage the advantage of automatic evaluation provided by F-UJI. The initial automatic evaluation provides concrete feedback for users to revise and enhance the datasets.  The final evaluation, also by automatic evaluation service,  can attest the revised dataset indeed fulfill the FAIR principles by passing all the evaluation metrics.
This approach is superior than the questionnaire-based evaluations that users' input to the evaluation has no ambiguities and can not lead to any biased evaluation results.

\todo{I am confused here. I expected that the final assessment will also need both auto+manual assessment together. It should be the same as the initial assessment.}

%Some helpful info: https://www.osti.gov/servlets/purl/1579323

%TODO: main points: 1) we develop HPC Ontology as standard metadata to annotate data, We use tarql to automatically convert csv to RDF (nt and json-ld formats).  add license, etc. 


%TODO: upload our datasets and models to existing websites. 

%two levels: 1) domain-level metadata, annotating entire csv files or AI model files 2) file-level (csv into RDF json-ld format)

\end{comment}

==> TEML'22 FAIRness-Extended-arXiv/relatedWork.tex <==
There are other schemes and proposals to promote open public data and make the data easy to use by others.  
Linked Open Data (LOD) refers to all data that is published on the Web according to a set of best practices \cite{Bizer2018}.  
Berners-Lee proposed Linked Open Data (LOD) principles\footnote{https://www.w3.org/DesignIssues/LinkedData.html} with four rules to prepare the web of open-linked data. 
A 5-star scoring system is provided to evaluate if the linked open data is truly open and easy for use.  
%These principles promotes the standardized data representation, propagating hyperlinks connected between data from different sources, and open data access through the Web. 
%Hasnain et. al. assess the FAIR Guiding Principles against the LOD principles and conclude that the FAIR principles cover a wider range of data whereas the LOD principles focus only the public open data\cite{hasnain2018assessing}.
%The FAIR principles have prompted many activities to improve the data FAIRness.

There are various FAIRness evaluations proposed to help improving data FAIRness.
The FAIRshake was developed to promote the FAIRification of data produced by biomedical research projects and enable the establishment of community driven FAIR metrics and rubrics paired with manual and automated FAIR assessments\cite{clarke2019fairshake}. 
Authors of the FAIR Guiding Principles use 14 FAIR metrics and the web interfaces for a semi-automated FAIR evaluation service\cite{wilkinson2019evaluating}.
Many activities from different research communities start to address the demand to apply FAIR principles in their datasets. 
Cuno et al. present the FAIR evaluation of datasets for stress detection systems\cite{cuno2020fair}.   
Lamprecht and the team study the need for FAIR research software\cite{lamprecht2020towards} and suggest revised terms in FAIR principles to cover the traits in research software.  

%\todo{What are the most FAIR datasets or models we have found so far? What do we learn from them}

%\todo{Summarize how this paper differs from related work}
